Complexity Classification of the Eight-Vertex Model

We prove a complexity dichotomy theorem for the eight-vertex model. For every setting of the parameters of the model, we prove that computing the partition function is either solvable in polynomial time or \#P-hard. The dichotomy criterion is explicit. For tractability, we find some new classes of problems computable in polynomial time. For \#P-hardness, we employ M\"{o}bius transformations to prove the success of interpolations.

==> 1intro-s.tex <==
\section{Introduction}\label{sec:intro}

There are two complementary motivations for this work, one
from physics, and one from the classification program for counting problems
in complexity theory.
From physics, there is a long history in the study of
various elegant models which define partition functions
that capture physical properties.
The eight-vertex model is one such model,
and it generalizes the six-vertex model. From
complexity theory,
we have made substantial progress in classifying counting
problems expressed as  \emph{sum-of-product}
computations in  all three frameworks: graph homomorphisms (GH),
counting constraint satisfaction problems (\#CSP),
and Holant problems. However,
the advances for GH and \#CSP have been far more conclusive
than for Holant problems: On the Boolean domain (where variables take
0-1 values), the  known complexity dichotomy for \#CSP
applies to all complex-valued
 constraint functions which need not be symmetric~\cite{cailuxia-2014},
but currently  the strongest Holant dichotomy without auxiliary
functions can only handle symmetric constraints~\cite{caiguowilliams13}.
%{cai-fu-guo-williams} for planar.
To classify Holant problems without the symmetry assumption,
currently we have to assume the presence of auxiliary functions.
 E.g., assuming all unary functions are present,
called Holant$^*$ problems, we have a dichotomy
that applies to symmetric as well as asymmetric
constraint functions~\cite{cailuxiastar}.
Beckens~\cite{Beckens-arXiv} recently proved an extension to a dichotomy
for Holant$^+$ problems, which assume the presence of
four unary functions including the  pinning functions
{\sc Is-Zero} and {\sc Is-One}
(which set a variable to 0 or 1).
If one only assumes the presence of
the two pinning functions, this is called  the Holant$^c$
problems.  The strongest known  Holant$^c$ dichotomies
are for symmetric complex-valued constraints~\cite{cai-huang-lu}, or
for  real-valued
constraints without symmetry assumption~\cite{cailuxia-2017}.
If one considers what tractable problems emerge
on planar graphs, again we have a full dichotomy
for Pl-\#CSP~\cite{cai:fu:plcsp}, but only for symmetric
constraints concerning Pl-Holant problems~\cite{cai-fu-guo-williams}.
%%
%% also GH Cai-Chen-Lu, general #CSP Cai-Chen, planar: cai-lu-xia, Guo-williams
% Cai-Fu... anything else?  spin systems?  Dyer-Greenhill, Bulatov-Grohe,
%Bulatov, Dyer-Richerby, Cai-Chen-Lu for nonnegative general domain #CSP
% check the Cai-Chen paper for others. Jerrum, Goldberg etc.
%for \#CSP cover for symmetric as well as asymmetric
%constraint functions, while the dichotomy for Holant problems
%on the Boolean domain only applies to symmetric constraints.
There are also several known dichotomies for GH and \#CSP
on domain size greater than $2$~\cite{Dyer-Greenhill,Bulatov-Grohe,Goldberg-Jerrum-Grohe-Thurley,Cai-Chen-Lu-forGH,
1-below-Bulatov-Dalmau,Bulatov,Dyer-Richerby,2-below,Cai-Chen-Lu-for-nonnegative-general-domain-CSP,Cai-Chen-generalCSP},
but very little is known for Holant problems.

% "1-below"
%A. A. Bulatov and V. Dalmau, Towards a dichotomy theorem for the counting constraint satisfaction problem, Inform. and Comput., 205 (2007), pp. 651--678
% "2-below"
%A. Bulatov, M. Dyer, L. A. Goldberg, M. Jalsenius, M. Jerrum, and D. Richerby, The complexity of weighted and unweighted #CSP, J. Comput. System Sci., 78 (2012), pp. 681--688,

Generally speaking, to handle constraint functions that are
not necessarily symmetric seems to be very challenging
for Holant problems.  The
%six-vertex model  and the
eight-vertex model can be
viewed as fundamental building blocks toward a full Holant dichotomy
on the Boolean domain without the symmetry restrictions.
Not only they are small arity cases
in such a theorem, they also present a pathway to overcome
some technical obstacles.
%such as the parity condition.

\input{8input-s}

In physics, the eight-vertex model  is
%considers a large number of oxygen and hydrogen atoms, and is
a generalization of
the six-vertex model, including models for water ice,
potassium dihydrogen phosphate KH$_2$PO$_4$ (KDP model of a ferroelectric)
and the Rys $F$ model of an antiferroelectric.
One can mathematically describe the  eight-vertex model as an orientation
problem on 4-regular graphs: Given a 4-regular graph $G = (V, E)$,
an orientation is an assignment of a direction to every $e \in E$.
An orientation is valid for the eight-vertex model
iff at every vertex the in-degree (and out-degree) is even.
This generalizes the six-vertex model where the in-degree (and out-degree)
is two and thus the orientation
is \emph{Eulerian}.  One can think of the valid configurations
in a eight-vertex model
as Eulerian orientations with possible sources and sinks.
The valid local configurations are illustrated in Figure~\ref{figure:8-vertexxx}.
The  energy $E$  of the system is determined by
eight parameters $\epsilon_1, \epsilon_2, \ldots, \epsilon_8$
associated with each type of the local configuration,
and $w_j = \exp\left(-\frac{\epsilon_j}{k_B T}\right)$
is called the  Boltzmann weight ($k_B$
 is Boltzmann's constant, and $T$ is the system's temperature).
If there are  $n_i$ sites in  local configuration type $i$,
 then
$E = n_1 \epsilon_1 + \ldots +  n_8  \epsilon_8$
is the total energy,
and the  partition function is $Z_{\rm Eight} = \sum e^{-E/k_BT}
= \sum \prod w_j^{n_j}$,
where the sum is  over all valid configurations.
This is a sum-of-product computation.
In our more general
definition (see Subsection~\ref{trac}) the 8 possible weights $w_j$
can be zero, and thus the six-vertex model is the special case
with $w_7=w_8=0$, disallowing the configurations 7 and 8.

Compared to the six-vertex model,  there are more
non-trivial tractable problems. Partly this is
 because the support of a
constraint function in the eight-vertex model can be an affine subspace
of dimension 3 (over ${\mathbb Z}_2$).
Some tractable problems are only revealed to be
so after surprising holographic transformations
$\left[\begin{smallmatrix}
1 & \frak{i} \\
\frak{i} & 1
\end{smallmatrix}\right]$
or
$\left[\begin{smallmatrix}
1 & 0 \\
0 & \sqrt[4]{\frak{i}}
\end{smallmatrix}\right]$. No previously known tractable classes
required such transformations.
More  tractable problems usually mean that
it is more challenging to prove a dichotomy.
Such a theorem says that there are no other tractable problems
beyond the ones already discovered (if \#P does not
collapse to P.)

We discover a connection for a class of
8-vertex models with \#CSP$^2$ problems,
which are a variant of  \#CSP
where every variable appears an even number of times.
%This is forced by the support structure of the
%constraint function in the 8-vertex model,
%and being an  \#CSP$^2$ problem there are more
Compared to \#CSP, there are more tractable problems
for \#CSP$^2$.  A crucial ingredient in our proof
is a recent \#CSP$^2$ dichotomy~\cite{cailuxia-2017} that is valid for
asymmetric signatures.
Our new tractable families for the 8-vertex model
also give new tractable families for the
so-called 2,4-spin Ising model on the lattice graph,
where the $(+/-)$ spins are on square faces, and
local interactions are among horizontal, vertical, two diagonals, and
all 4 neighbors.

A new contribution of this work is to use
M\"{o}bius transformations
 ${\mathfrak z} \mapsto
\frac{a {\mathfrak z} + b}{c {\mathfrak z} + d}$
to prove \#P-hardness.
Typically to prove some problem \#P-hard by
interpolation, we want to prove that certain
quantities (such as eigenvalues)
are not roots of unity, lest the iteration repeat after
a bounded number of steps.
We usually establish this property by showing that
we can produce these quantities of norm $\ne 1$.
However in this paper, there are settings where this is
impossible. In this case we prove that
the constraint functions define certain M\"{o}bius transformations
that map the unit circle to
 unit circle on $\mathbb{C}$. By exploiting the mapping
properties we can
obtain a suitable M\"{o}bius transformation which generates a group of
infinite order. Hence even though they only produce
quantities of complex norm 1, they nevertheless can be guaranteed
not to repeat.
This allows us to show that
our interpolation proof succeeds.



==> 2-4-spin-Ising-s.tex <==
$\mathbf{Problems:}$ 2,4-spin  Ising model on lattice graph.

There is a well known correspondence between the eight-vertex model
 on the lattice graph on the one hand,
and a 2,4-spin  Ising model on the other hand,
where the variables of the  Ising model are the square faces
of the lattice graph.
Suppose we assign a spin $\sigma_{i,j}$
to the $(i,j)$-square face of an $N \times N$ lattice
(with boundary wrapping around forming a torus).
Each  spin $\sigma_{i,j}$ takes values $\pm 1$.
There are 5 local interactions between these spins.

In the following $J_h, J_v, J, J', J''$ are constants.
Between $\sigma_{i,j}$ and  $\sigma_{i+1,j}$,
there is a (horizontal neighbor) ``edge function'':
$f_h (\sigma, \sigma') = e^{-J_h \sigma \cdot \sigma'}$.
Thus if $\sigma_{i,j} = \sigma_{i+1,j}$ then the output value is
$e^{-J_h}$, otherwise, it is $e^{J_h}$.
As a signature matrix, $M(f_h) =
\left[\begin{smallmatrix}
e^{-J_h} & e^{J_h}\\
e^{J_h} & e^{-J_h}
\end{smallmatrix}\right]$.

Similarly between $\sigma_{i,j}$ and  $\sigma_{i,j+1}$,
there is a (vertical  neighbor) ``edge function'':
$\left[\begin{smallmatrix}
e^{-J_v} & e^{J_v}\\
e^{J_v} & e^{-J_v}
\end{smallmatrix}\right]$.
Between
 $\sigma_{i+1,j}$ and  $\sigma_{i,j+1}$,
there is one diagonal ``edge function'' $f_d =
\left[\begin{smallmatrix}
e^{-J} & e^{J}\\
e^{J} & e^{-J}
\end{smallmatrix}\right]$;
and  between $\sigma_{i,j}$ and $\sigma_{i+1,j+1}$,
there is another  diagonal ``edge function'' $f_d' =
\left[\begin{smallmatrix}
e^{-J'} & e^{J'}\\
e^{J'} & e^{-J'}
\end{smallmatrix}\right]$.
Finally there is a 4-ary function,
$f_4(\sigma_{i,j}, \sigma_{i,j+1}, \sigma_{i+1,j}, \sigma_{i+1,j+1})
= e^{-J''p}$,
where $p$ is the product $\sigma_{i,j} \sigma_{i,j+1}  \sigma_{i+1,j}
\sigma_{i+1,j+1}$.

The  partition function of this 2,4-spin Ising model
is the sum over all spins $\sigma_{i,j} = \pm 1$
of the product
\[\prod_{i,j} f_h(\sigma_{i,j}, \sigma_{i+1,j})
f_v (\sigma_{i,j}, \sigma_{i,j+1})
f_d(\sigma_{i,j+1}, \sigma_{i+1,j})
f_d'(\sigma_{i,j}, \sigma_{i+1,j})
f_4(\sigma_{i,j}, \sigma_{i,j+1}, \sigma_{i+1,j}, \sigma_{i+1,j+1}).\]

It turns out that there is two-to-one exact correspondence
between spin assignments on $\sigma_{i,j}$
and orientations for the eight-vertex model.
The parameters are related as follows:
\begin{eqnarray*}
\epsilon_1 &=& -J_h - J_v - J - J' - J''\\
\epsilon_2 &=& +J_h + J_v - J - J' - J''\\
\epsilon_3 &=& -J_h + J_v + J + J' - J''\\
\epsilon_4 &=& +J_h - J_v + J + J' - J''\\
\epsilon_5=\epsilon_6 &=& \hspace{.6in} +~ J -  J' + J''\\
\epsilon_7=\epsilon_8 &=& \hspace{.6in} -~ J +  J' + J''
\end{eqnarray*}

By our theorem for the eight-vertex model,
this implies that, e.g.,
the 2,4-spin Ising model on the lattice graph
is polynomial time computable
if $(J_h, J_v, J, J', J'') =
\frac{\pi {\frak i}}{4}
(0, 2, -1, -1, 0)$.

%%% was e^{.... e_1, e_2, ... e_8, for affine
%  only e^{\epsilon_2} = e^{\epsilon_4} =-1, rest all = 1.
% chose: \epsilon_2 =\pi i, \epsilon_4 = -\pi i.
% rest all \epsilon_1, .. \epsilon__8 =0.




==> 2-4-spin-Ising.tex <==
$\mathbf{Problems:}$ 2,4-spin  Ising model on lattice graph.

There is a well known correspondence between the eight-vertex model
 on the lattice graph on the one hand,
and a 2,4-spin  Ising model on the other hand,
where the variables of the  Ising model are the square faces
of the lattice graph.
Suppose we assign a spin $\sigma_{i,j}$
to the $(i,j)$-square face of an $N \times N$ lattice
(with boundary wrapping around forming a torus).
Each  spin $\sigma_{i,j}$ takes values $\pm 1$.
There are 5 local interactions between these spins.

In the following $J_h, J_v, J, J', J''$ are constants.
Between $\sigma_{i,j}$ and  $\sigma_{i+1,j}$,
there is a (horizontal neighbor) ``edge function'':
$f_h (\sigma, \sigma') = e^{-J_h \sigma \cdot \sigma'}$.
Thus if $\sigma_{i,j} = \sigma_{i+1,j}$ then the output value is
$e^{-J_h}$, otherwise, it is $e^{J_h}$.
As a signature matrix, $M(f_h) =
\left[\begin{smallmatrix}
e^{-J_h} & e^{J_h}\\
e^{J_h} & e^{-J_h}
\end{smallmatrix}\right]$.

Similarly between $\sigma_{i,j}$ and  $\sigma_{i,j+1}$,
there is a (vertical  neighbor) ``edge function'':
$M(f_v)=\left[\begin{smallmatrix}
e^{-J_v} & e^{J_v}\\
e^{J_v} & e^{-J_v}
\end{smallmatrix}\right]$.
Between
 $\sigma_{i+1,j}$ and  $\sigma_{i,j+1}$,
there is one diagonal ``edge function'' $f_d =
\left[\begin{smallmatrix}
e^{-J} & e^{J}\\
e^{J} & e^{-J}
\end{smallmatrix}\right]$;
and  between $\sigma_{i,j}$ and $\sigma_{i+1,j+1}$,
there is another  diagonal ``edge function'' $f_d' =
\left[\begin{smallmatrix}
e^{-J'} & e^{J'}\\
e^{J'} & e^{-J'}
\end{smallmatrix}\right]$.
Finally there is a 4-ary function,
$f_4(\sigma_{i,j}, \sigma_{i,j+1}, \sigma_{i+1,j}, \sigma_{i+1,j+1})
= e^{-J''p}$,
where $p$ is the product $\sigma_{i,j} \sigma_{i,j+1}  \sigma_{i+1,j}
\sigma_{i+1,j+1}$.

The  partition function of this 2,4-spin Ising model
is the sum over all spins $\sigma_{i,j} = \pm 1$
of the product
\[\prod_{i,j} f_h(\sigma_{i,j}, \sigma_{i+1,j})
f_v (\sigma_{i,j}, \sigma_{i,j+1})
f_d(\sigma_{i,j+1}, \sigma_{i+1,j})
f_d'(\sigma_{i,j}, \sigma_{i+1,j})
f_4(\sigma_{i,j}, \sigma_{i,j+1}, \sigma_{i+1,j}, \sigma_{i+1,j+1}).\]

It turns out that there is two-to-one exact correspondence
between spin assignments on $\sigma_{i,j}$
and orientations for the eight-vertex model.
The parameters are related as follows:
\begin{eqnarray*}
\epsilon_1 &=& -J_h - J_v - J - J' - J''\\
\epsilon_2 &=& +J_h + J_v - J - J' - J''\\
\epsilon_3 &=& -J_h + J_v + J + J' - J''\\
\epsilon_4 &=& +J_h - J_v + J + J' - J''\\
\epsilon_5=\epsilon_6 &=& \hspace{.6in} +~ J -  J' + J''\\
\epsilon_7=\epsilon_8 &=& \hspace{.6in} -~ J +  J' + J''
\end{eqnarray*}

By our theorem for the eight-vertex model,
this implies that, e.g.,
the 2,4-spin Ising model on the lattice graph
is polynomial time computable
if $(J_h, J_v, J, J', J'') =
\frac{\pi {\frak i}}{4}
(0, 2, -1, -1, 0)$.

%%% was e^{.... e_1, e_2, ... e_8, for affine
%  only e^{\epsilon_2} = e^{\epsilon_4} =-1, rest all = 1.
% chose: \epsilon_2 =\pi i, \epsilon_4 = -\pi i.
% rest all \epsilon_1, .. \epsilon__8 =0.




==> 2pre-s.tex <==
\section{Preliminaries}

\subsection{Definitions and Notations}
In the present paper, $\frak{i}$ denotes a square root of $-1$, i.e., $\frak{i}^2=-1$.
$\alpha$ denotes a square root of $\frak{i}$, i.e., $\alpha^2=\frak{i}$.
Let $\mathbb{N} = \{0,1,2,\ldots\}$,
$H=\frac{1}{\sqrt{2}}
\left[\begin{smallmatrix}
1 & 1 \\
 1 & -1
\end{smallmatrix}\right]
$, $Z=\frac{1}{\sqrt{2}} \left[\begin{smallmatrix}
1 & 1 \\
\mathfrak{i} & -\mathfrak{i}
\end{smallmatrix}\right]$.


A constraint function $f$ of arity $k$
is a map $\{0,1\}^k  \rightarrow \mathbb{C}$.
Fix a set $\mathcal{F}$ of constraint functions. A signature grid
$\Omega=(G, \pi)$
 is a tuple, where $G = (V,E)$
is a graph, $\pi$ labels each $v\in V$ with a function
$f_v\in\mathcal{F}$ of arity ${\operatorname{deg}(v)}$,
and the incident edges
$E(v)$ at $v$ with input variables of $f_v$.
% Each
%$f_v$ maps
%$\{0, 1\}^{\operatorname{deg}(v)}$ to $\mathbb{C}$.
 We consider all 0-1 edge assignments $\sigma$,
each gives an evaluation
$\prod \limits_{v\in V}f_v(\sigma|_{E(v)})$, where $\sigma|_{E(v)}$
denotes the restriction of $\sigma$ to $E(v)$. The counting problem on the instance $\Omega$ is to compute
$$\operatorname{Holant}_{\Omega}(\mathcal{F})=\sum\limits_{\sigma:E\rightarrow\{0, 1\}}\prod_{v\in V}f_v(\sigma|_{E(v)}).$$
The Holant problem parameterized by the set $\mathcal{F}$ is denoted by Holant$(\mathcal{F})$.
We also write  Holant$(\mathcal{F}, f)$
for Holant$(\mathcal{F} \cup \{f\})$.
A constraint function is also called a signature.
%If $\mathcal{F}=\{f\}$ is a single set, for simplicity, we write $\{f\}$ as $f$ directly and also write $\{f\} \cup \{g\}$ as $f\cup g$.
%When $G$ is a planar graph, the corresponding signature grid is called a planar grid.
%$\PlHolant(\mathcal{F})$ denotes its restriction to planar graphs $G$.
We use Holant$(\mathcal{F}|\mathcal{G})$ to denote the Holant problem over signature grids with a bipartite graph $H = (U,V,E)$,
where each vertex in $U$ or $V$ is assigned a signature in $\mathcal{F}$ or $\mathcal{G}$
respectively.
\#CSP$(\mathcal{F})$
can be defined as Holant$(\mathcal{EQ}|\mathcal{F})$ % $\holant{\mathcal{EQ}}{\mathcal{F}}$,
where $\mathcal{EQ} = \{{=}_1, {=}_2, \dotsc\}$ is the set of \textsc{Equality} signatures.
Similarly,
\#CSP$^2(\mathcal{F})$
can be defined as Holant$(\mathcal{EQ}_2|\mathcal{F})$ % $\holant{\mathcal{EQ}}{\mathcal{F}}$,
where $\mathcal{EQ}_2 = \{{=}_2, {=}_4, \dotsc\}$ is the set of \textsc{Equality} signatures
of even arities, i.e., every variable appears an even number of times.

A function $f$ of arity $k$ can be represented as a vector 
 by listing its values in lexicographical order as  in a truth table.
Also a signature $f$ of arity 4 has the signature matrix
$M(f)=M_{x_1x_2, x_3x_4}(f) = \left[\begin{smallmatrix}
f_{0000} & f_{0001} & f_{0010} & f_{0011}\\
f_{0100} & f_{0101} & f_{0110} & f_{0111}\\
f_{1000} & f_{1001} & f_{1010} & f_{1011}\\
f_{1100} & f_{1101} & f_{1110} & f_{1111}
\end{smallmatrix}\right]
.$
If $\{i,j,k,\ell\}$ is a permutation of $\{1,2,3,4\}$,
then the $4 \times 4$ matrix $M_{x_ix_j, x_kx_{\ell}}(f)$ lists the 16 values
 with row  index $x_ix_j \in\{0, 1\}^2$
and column index
$x_kx_{\ell} \in\{0, 1\}^2$ in lexicographic order.
% which
%%$\mathbb{C}^{2^{k}}$, or as a tensor in $(\mathbb{C}^2)^{\otimes k}$, or as a matrix in $\mathbb{C}^{2^{k_1}}\times \mathbb{C}^{2^{k_2}}$
%if we partition the $k$ variables to two parts,  where $k_1+k_2=k$.
%A function is symmetric if its value depends only
%on the Hamming weight of its input.
%A symmetric function $f$ on $k$ Boolean variables can
%be expressed as
%$[f_0, f_1, \ldots, f_k]$,
%where $f_w$ is the value of $f$ on inputs of Hamming weight $w$.
%For example, $(=_k)$ is the {\sc Equality} signature $[1, 0, \ldots, 0, 1]$
%(with $k-1$ 0's) of arity $k$.
A binary signature $g$ has the signature matrix
$M(g)=\left[\begin{smallmatrix}
 g_{00} & g_{01}\\
g_{10} & g_{11}
\end{smallmatrix}\right]
.$
We use $\neq_2$ to denote binary {\sc Disequality} function $(0, 1, 1, 0)^T$
indexed by $x_1x_2\in\{0, 1\}^2$ and its matrix form is $\left[\begin{smallmatrix}
0 & 1 \\
 1 & 0
\end{smallmatrix}\right]$. Note that
$N=
\left[\begin{smallmatrix}
0 & 1 \\
 1 & 0
\end{smallmatrix}\right]
\otimes
\left[\begin{smallmatrix}
0 & 1 \\
 1 & 0
\end{smallmatrix}\right]
=
\left[\begin{smallmatrix}
 0 & 0 & 0 & 1 \\
 0 & 0 & 1 & 0 \\
 0 & 1 & 0 & 0 \\
 1 & 0 & 0 & 0 \\
\end{smallmatrix}\right]$, i.e.,
 $N$ is the double {\sc Disequality} in parallel,
which is the function of connecting two pairs of edges by $(\not =_2)$.
The support of a function $f$ is the set of inputs on which $f$ is nonzero.

The eight-vertex model is the Holant problem Holant$(\neq_2 \mid f)$ where
$f$ is a 4-ary signature with the signature matrix
$M(f)=\left[\begin{smallmatrix}
a & 0 & 0 & b\\
0 & c & d & 0\\
0 & w & z & 0\\
y & 0 & 0 & x\\
\end{smallmatrix}\right]$.
 We call $(a, x)$  the outer pair of $f$, $ (b, y), (c, z), (d, w)$  the inner pairs of $f$,
$\left[\begin{smallmatrix}
a & b\\
y & x\\
\end{smallmatrix}\right]$  the outer matrix of $f$ and
$\left[\begin{smallmatrix}
 c & d\\
 w & z
\end{smallmatrix}\right]$  the inner matrix of $f$.
Denote the 3 inner pairs of
 ordered complementary strings
%%%%%%%%%%JYC, since in lm 4.1 we use alpha ...
%for actual entry values. i change them. al--> la, be --> mu , gamma --> nu
%%%%%%%%%
% by $\alpha = 0011, \overline{\alpha} = 1100$,
%$\beta = 0110, \overline{\beta} = 1001$, and $\gamma = 0101, \overline{\gamma}
%= 1010$.
%The support of $f$ is the union of the pairs $(\alpha, \overline{\alpha})$,
%$(\beta, \overline{\beta})$ and $(\gamma, \overline{\gamma})$,
%on which $f$ has values
%$(a,x), (b,y)$ and $(c,z)$.
%If $f$ has the same value in  a pair,
% say $a=x$ on $\alpha$ and $\overline{\alpha}$,
% we say it is a twin.
%%%%%%%%%%%%%%%%%%%%%%
 by $\lambda = 0011, \overline{\lambda} = 1100$,
$\mu = 0110, \overline{\mu} = 1001$, and $\nu = 0101, \overline{\nu}
= 1010$.
The permutation group $S_4$ on $\{x_1, x_2, x_3, x_4\}$
induces a group action on $\{s \in \{0, 1\}^4
\mid {\rm wt}(s) =2\}$ of size 6.
This is a faithful representation of $S_4$ in $S_6$.
% Every nontrivial $\sigma \in S_4$
%induces a nontrivial. For, if j=sigma(i) \not =i, then there is
% a string s: s_i =0, s_j = 1, rest have equal wt, so total wt 2.
%%and sigma(s) \not = s.
Since the action of $S_4$ preserves complementary pairs,
%strings,
this group action has nontrivial blocks of imprimitivity,
%namely $\{\{0011,1100\}, \{0110,1001\}, \{0101,1010\}\}$.
namely $\{A,B,C\} =
\{\{\lambda, \overline{\lambda}\},
\{\mu, \overline{\mu}\}, \{\nu, \overline{\nu}\}\}$.
The action on the blocks is a homomorphism of $S_4$ onto
$S_3$, i.e., we can
permute the blocks arbitrarily by permuting the variables $\{x_1, x_2, x_3, x_4\},$
 with kernel $K = \{1, (12)(34), (13)(24), (14)(23)\}$.
In particular one can calculate that the subgroup
$S_{\{2,3,4\}} = \{1, (23), (34), (24), (243), (234)\}$
maps to $\{1, (AC), (BC), (AB), (ABC), (ACB)\}$.
%%% actually even more explicit:
% 1, (ac)(a'c'), (bc)(b'c'), (ab)(a'b'), (abc)(a'b'c'), (acb)(a'c'b')
%To summerize,
By a permutation from $S_4$,
we may permute the matrix $M(f)$
by any permutation on the values
$\{b, c, d\}$ with the corresponding permutation on $\{y, z, w\}$,
and moreover we can further flip
%within
an even number
of pairs $(b, y)$, $(c, z)$
and $(d, w)$.
In particular, we can
arbitrarily reorder the  three rows in
$\left[\begin{smallmatrix}
b & y \\
c & z \\
d & w
\end{smallmatrix}\right]$, and
we can also reverse the order of
 arbitrary two rows together.
 In the following, when we say by the symmetry of $\{(b, y), (c, z), (d, w)\}$,
 it means this group action.



%$\plholant{\mathcal{F}}{\mathcal{G}}$ denotes its planar restriction.
%$\plholant{\mathcal{F}}{\mathcal{G}}$ denotes the Holant problem over signature grids with a planar bipartite graph.
%Counting constraint satisfaction problems (\#CSP)
%can be defined as Holant$(\mathcal{EQ}|\mathcal{G}$% $\holant{\mathcal{EQ}}{\mathcal{F}}$,
%where $\mathcal{EQ} = \{{=}_1, {=}_2, {=}_3, \dotsc\}$ is the set of \textsc{Equality} signatures of all arities;
%For any positive integer $d$,
%the problem \#CSP$^d(\mathcal{F})$ is the same as \#CSP$(\mathcal{F})$ except that every variable appears a multiple of $d$ times.
%Thus,
%$\#\operatorname{CSP}^d(\mathcal{F}) \equiv_T \operatorname{Holant}(\mathcal{EQ}_d){\mathcal{F}}$,
%where $\mathcal{EQ}_d = \{{=}_d, {=}_{2 d}, {=}_{3 d}, \dotsc\}$ is the set of \textsc{Equality} signatures of arities that are multiples of $d$.
%For $d=1$, we have just \#CSP problems. For $d=2$,
%these are \#CSP problems where every variable appears an even number of times.
% that is $({=}_k)=(1, 0, \cdots, 0, 1)$.
%Similarly, its planar restriction
%its planar restriction
 %$\PlCSP(\mathcal{F})$ is $\plholant{\mathcal{EQ}}{\mathcal{F}}$.

%We can treat the support of $f$ as a relation or a $0,1$-valued function.
%%% JYC not used. i think


%An instance of $\CSP(\mathcal{F})$ is presented
%as a bipartite graph.
%There is one node for each variable and for each occurrence
%of constraint functions respectively.
%Connect a constraint node to  a variable node if the
%variable appears in that occurrence
%of constraint, with a labeling on the edges
%for the order of these variables.
%This bipartite graph is also known as the \emph{constraint graph}.
%If we attach each variable node with an \textsc{Equality} function,
%and consider every edge as a variable, then
%the \#CSP is just the Holant problem on this bipartite graph.
%hus
%$\CSP(\mathcal{F}) \equiv_T \holant{\mathcal{EQ}}{\mathcal{F}}$,
%where $\mathcal{EQ} = \{{=}_1, {=}_2, {=}_3, \dotsc\}$ is the set of \textsc{Equality} signatures of all arities, that is ${=}_k=(1, 0, \cdots, 0, 1)$.
%y restricting to planar constraint graphs,
%we have the planar \#CSP framework,
%which we denote by $\PlCSP$.%


%For $T \in {\rm GL}_2({\mathbb{C}})$
% and a signature $f$ of arity $n$, written as
%a column vector  $f \in \mathbb{C}^{2^n}$, we denote by
%$T^{-1}f = (T^{-1})^{\otimes n} f$ the transformed signature.
%  For a signature set $\mathcal{F}$,
%define $T^{-1} \mathcal{F} = \{T^{-1}f \mid  f \in \mathcal{F}\}$.
%For signatures written as
% row vectors we define $\mathcal{F} T$ similarly.
%Whenever we write $T^{-1} f$ or $T^{-1} \mathcal{F}$,
%we view the signatures as column vectors;
%similarly for $f T$ or $\mathcal{F} T$ as row vectors.
%
%
%Let $T \in {\rm GL}_2({\mathbb{C}})$.
%The holographic transformation defined by $T$ is the following operation:
%given a signature grid $\Omega = (H, \pi)$ of Holant$(\mathcal{F}|\mathcal{G})$,
%for the same bipartite graph $H$,
%we get a new signature grid $\Omega' = (H, \pi')$ of Holant$(\mathcal{F} T|T^{-1} \mathcal{G})$ by replacing each signature in
%$\mathcal{F}$ or $\mathcal{G}$ with the corresponding signature in $\mathcal{F} T$ or $T^{-1} \mathcal{G}$.
For Holant$(\neq_2|f)$,
 we say that $f$ is
$\mathscr{C}$-transformable if there exists $T \in {\rm GL}_2({\mathbb{C}})$
such that we have both
  $(\neq_2)T^{\otimes 2} \in  \mathscr{C}$ and $(T^{-1})^{\otimes 4} f
\in \mathscr{C}$.
%For  $\mathcal{G} = \mathcal{EQ}$,
%Holant${\mathcal{EQ}}{\mathcal{F}}  \equiv_T \#\operatorname{CSP}(\mathcal{F})$,
%we say that $\mathcal{F}$ is
%$\mathscr{C}$-transformable for \#$\operatorname{CSP}$.
%We define similarly for \#$\operatorname{CSP}^d$ when   $\mathcal{G} = \mathcal{EQ}_d$.
%\end{definition}
Notice that if
$\operatorname{Holant}(\mathscr{C}|\mathscr{C})$ is tractable, and
$f$
is $\mathscr{C}$-transformable,
then $\operatorname{Holant}(\neq_2 | f)$ is tractable
by a holographic transformation.








%If we have a  binary signature $(0, 1, x, 0) \in \mathcal{F}$
%in addition to $f \in \mathcal{F}$, we may connect it
%to some variable of $f$ using $\neq_2$.
%% $f$ by connecting a binary signature $(0, 1, x, 0)$
%%to some variable of $f$ using $\neq_2$.
%For example, when we connect the first variable of $(0, 1, x, 0)$ to $x_1$ of $f$ by $\neq_2$, we get the signature $g$ with the signature matrix
%$M_{x_1x_2, x_4x_3}(g)=
%\left[\begin{smallmatrix}
%xf_{0000} & xf_{0010} & xf_{0001} & xf_{0011}\\
%xf_{0100} & xf_{0110} & xf_{0101} & xf_{0111}\\
%f_{1000} & f_{1010} & f_{1001} & f_{1011}\\
%f_{1100} & f_{1110} & f_{1101} & f_{1111}
%\end{smallmatrix}\right]$.
%When we connect the second variable of $(0, 1, x, 0)$ to $x_1$ of $f$ by $\neq_2$, we will get the signature $h$ with the signature matrix
%$M_{x_1x_2, x_4x_3}(h)=
%\left[\begin{smallmatrix}
%f_{0000} & f_{0010} & f_{0001} & f_{0011}\\
%f_{0100} & f_{0110} & f_{0101} & f_{0111}\\
%xf_{1000} & xf_{1010} & xf_{1001} & xf_{1011}\\
%xf_{1100} & xf_{1110} & xf_{1101} & xf_{1111}
%\end{smallmatrix}\right]$.

%A signature $f$ of arity $k$ is degenerate if there exist unary signatures $u_i\in\mathbb{C}^2$ for
%$1\leq i\leq k$ such that
%$f=\otimes_{i=1}^{k}u_i$. Replacing a degenerate  signature by the corresponding unary signatures
%$u_i$ does not change
%the Holant value.

%Replacing a signature
%$f\in\mathcal{F}$ by a constant multiple $cf$, where $c\neq 0$, does not change
%the complexity of Holant$(F)$. It introduces a global nonzero
%factor to Holant$_{\Omega}$.
%
%To introduce the idea of holographic reductions, it is convenient to consider bipartite graphs. For a
%general graph, we can always transform it into a bipartite graph while preserving the Holant value. For
%each edge in the graph, we replace it by a path of length two. Each new vertex is assigned the binary
%{\sc Equality} signature $(=_2) = [1, 0, 1]$.
%
%For a 2-by-2 matrix $T$ and a signature $f$ of arity $k$,
%the holographic transformation of $f$ is $Tf = T^{\otimes k} f$.
%For a signature set $\mathcal{F}$, define
%$T\mathcal{F}=\{Tf \mid f\in\mathcal{F} \}$.
%We similarly define $\mathcal{F}T$, where $f \in \mathcal{F}$
%are written as row vectors.
% Whenever we write $T^{\otimes n}f$ or $T\mathcal{F}$,
%(resp., $fT^{\otimes n}$ or $\mathcal{F}T$)  we view
% the signatures as column (resp., row) vectors.
% We use Holant$(\mathcal{R}| \mathcal{G})$
% to denote the Holant problem on bipartite graphs
%$H =(U, V,E)$, where each vertex in $U$ or $V$ is assigned a signature in $\mathcal{R}$ or $\mathcal{G}$, respectively. Let $T$ be an
%invertible 2-by-2 matrix. The holographic transformation defined by $T$ is the following operation: given
%a signature grid $\Omega$ with underlying graph $H$, we create a new grid $\Omega'$ such that the graph is still $H$, and
%any functions $f$ on the left (or $g$ on the right) is replaced by $fT^{\otimes n}$ (or $(T^{-1})^{\otimes n}g$) where $n$ and $m$ are
%arities of $f$ and $g$.
%The six-vertex  model is equivalent to Holant$(\neq_2|f)$, where $f$
%has the signature matrix
%$M_{x_1x_2, x_4x_3}(f)=
%\left[\begin{smallmatrix}
%0 & 0 & 0 & a\\
%0 & b & c & 0\\
%0 & a & y & 0\\
%x & 0 & 0 & 0\\
%\end{smallmatrix}\right]$.
\subsection{Gadget Construction}\label{subsec:Gadget-Construction}
An  $\mathcal{F}$-gate is a signature grid with a set of dangling edges $D$
and vertices labeled by signatures from $\mathcal{F}$.
It defines a function of arity $|D|$ in a naturally way:
For any assignment $D \rightarrow \{0, 1\}$,
the output is the Holant sum.
We say a signature $g$ is \emph{constructible} or \emph{realizable} from a signature set $\mathcal{F}$
if $g$ is the function defined by an  $\mathcal{F}$-gate.
If $g$ is realizable from $\mathcal{F}$,
then   Holant$(\mathcal{F}, g)$ $\leq^p_T$
  Holant$(\mathcal{F})$.



Doing binary modification to the variable $x_i$ of $f$ using the binary signature
$g(x_1, x_2)=(g_{00}, g_{01}, g_{10}, g_{11})=(0, 1, t, 0)^T$
means connecting the variable $x_i$ of $f$ to the variable $x_2$ of $g$ by $\neq_2$.
For example, by doing binary modification to the variable $x_1$ of $f$ using the binary signature
$(0, 1, t, 0)^T$ we get the signature $f'$ whose signature matrix is
\[M(f')=\left[\begin{smallmatrix}
f_{0000} & f_{0001} & f_{0010} & f_{0011}\\
f_{0100} & f_{0101} & f_{0110} & f_{0111}\\
tf_{1000} & tf_{1001} & tf_{1010} & tf_{1011}\\
tf_{1100} & tf_{1101} & tf_{1110} & tf_{1111}\\
\end{smallmatrix}\right].\]
%The reduction is simple.
%Given an instance of $\PlHolant(\mathcal{F}, g)$,
%by replacing every occurrence of $g$ by the $\mathcal{F}$-gate,
%we get an instance of $\PlHolant(\mathcal{F})$.
%Since the signature of the $\mathcal{F}$-gate is $g$,
%the Holant values for these two signature grids are identical. There are two common gadgets we will use in this paper.

%When a gadget has an asymmetric signature,
%we place a diamond on the edge corresponding to the first input.
%The remaining inputs are ordered counterclockwise around the vertex.




\subsection{Tractable Signatures}\label{trac}

We use $\mathscr{P}, \mathscr{A}, \alpha\mathscr{A}, \mathscr{L}$
 to denote four fundamental classes of tractable signatures.
 % are known to be tractable for \#CSP$^2$ \cite{cailuxia-2017, wang-lin-2016}.
%Moreover, $\mathscr{P}, \mathscr{A}$ are known to be tractable for \#CSP \cite{cailuxia-2014}.
% The classes $\mathscr{P}, \mathscr{A}, \widehat{\mathscr{M}}$ are
%identified as tractable for Pl-\#CSP \cite{Guo-Williams}.
%The support of a signature in $\mathscr{A}$ is an affine linear space over $\mathbb{Z}_2$.
A signature $f(x_1, \ldots, x_n)$ of arity $n$
is in $\mathscr{A}$ if it has the form
 $\lambda \cdot \chi_{A X = 0} \cdot {\frak i} ^{Q(X)},$
 where $\lambda \in \mathbb{C}$,
 $X = (x_1, x_2, \dotsc, x_n, 1)$,
 $A$ is a matrix over $\mathbb{Z}_2$,
 %$\mathbf{v}_j$ is a vector over $\mathbb{Z}_2$,
 $Q(x_1, x_2, \ldots, x_n)\in \mathbb{Z}_4[x_1, x_2, \ldots, x_n]$
is a quadratic (total degree at most 2) multilinear polynomial
 with the additional requirement that the coefficients of all
 cross terms are even,
 %i.e.,
 %$Q$ has the form
 %\[Q(x_1, x_2, \ldots, x_n)=a_0+\displaystyle\sum_{k=1}^na_kx_k+\displaystyle\sum_{1\leq i<j\leq n}2b_{ij}x_ix_j,\]
 and $\chi$ is a 0-1 indicator function
 such that $\chi_{AX = 0}$ is~$1$ iff $A X = 0$.
%For an $n$-ary nonzero signature $f\in\mathscr{A}$ whose support has dimension $k \ge 0$, let $X=\{x_{i_1}, x_{i_2}, \ldots, x_{i_k}\}$
%be a set of free variables for its support, then the compressed signature $\underline{f_X}$ of $f$ for $X$ is a $k$-ary
%signature and $\underline{f_X}(x_{i_1}, x_{i_2}, \ldots, x_{i_k})=f(x_1, x_2, \ldots, x_n)$, where $(x_1, x_2, \ldots, x_n)\in {\rm supp}(f)$.
%Moreover, after a nonzero scalar, all the nonzero entries of an affine signature are  powers of $\frak{i} = \sqrt{-1}$.
%Thus nonzero entries of an affine signature have the same norm.
Problems defined by $\mathscr{A}$ are tractable~\cite{cai:chen:ll}.
% essentially by Gauss sums
%\cite{cai:chen:ll}.
The signatures in $\mathscr{P}$ are tensor products of signatures whose supports are among two complementary
bit vectors. An $n$-ary signature $f\in\alpha\mathscr{A}$
iff $\left[\begin{smallmatrix}
1 & 0\\
0 & \alpha
\end{smallmatrix}\right]^{\otimes n}f\in\mathscr{A}$.
The problems in $\alpha\mathscr{A}$
 are tractable for \#CSP$^2$  by the holographic transformation.
 And Problems defined by $\mathscr{L}$ are tractable essentially by a local holographic transformation
\cite{cailuxia-2017}.
%\paragraph{Transformable}

%An important definition involving a holographic transformation is the notion of a signature set being transformable.

%\begin{definition} \label{def:prelim:trans}
% We say a pair of signature sets $(\mathcal{G}, \mathcal{F})$
%is $\mathscr{C}$-transformable for  Holant${\mathcal{G}}{\mathcal{F}}$
%%and $\plholant{\mathcal{G}}{\mathcal{F}}$
% if there exists $T \in \mathbf{GL}_2(\mathbb{C})$ such that
%$\mathcal{G}T \subseteq  \mathscr{C}$ and $T^{-1} {\mathcal{F}}
%\subseteq \mathscr{C}$.


%\begin{theorem}\cite{cailuxia-2014}\label{csp:dichotomy}
%Let $\mathcal{F}$ be any set of complex-valued signatures in Boolean variables. Then $\operatorname{\#CSP}(\mathcal{F})$
%is \#$\operatorname{P}$-hard unless
%$\mathcal{F}\subseteq\mathscr{A}$ or
%$\mathcal{F}\subseteq\mathscr{P}$,
%  in which case the problem is computable in polynomial time.
%\end{theorem}

Lin and Wang proved the following lemma (Lemma 3.4
in~\cite{wang-lin-2016}),
which says that one can always reduce a signature to its tensor power.
We will only need a special case; for the  convenience of readers we
state it below with a short proof.

\begin{lemma}[Lin-Wang]\label{lm:Lin-Wang}
For any set of signatures $\mathcal{F}$,
and a signature $f$, 
\[\operatorname{Holant}(\mathcal{F}, f)
\leq_{\rm T}^p
\operatorname{Holant}(\mathcal{F}, f^{\otimes 2}).\]
\end{lemma}
\begin{proof}
We ask the question: Is there a signature
grid $\Omega$ for $\operatorname{Holant}(\mathcal{F}, f)$
in which $f$ appears an odd number of times,
and the value
$\operatorname{Holant}_{\Omega}(\mathcal{F}, f)$ is nonzero?
If the answer is no, then here is a simple reduction:
For any input signature
grid $\Omega$ for $\operatorname{Holant}(\mathcal{F} ,f)$,
if  $f$ appears an odd number of times,
then $\operatorname{Holant}_{\Omega}(\mathcal{F} ,f) =0$,
otherwise, pair up occurrences of $f$ two at a time and 
replace them by one copy of $f^{\otimes 2}$.

Now suppose the answer is yes, and let
$c = \operatorname{Holant}_{\Omega_0}
(\mathcal{F}, f) \not =0$, where $\Omega_0$ is 
a signature grid in which $f$ appears $2k+1$ times.
Replace $2k$ occurrences of $f$ in $\Omega_0$ 
by $k$ copies of $f^{\otimes 2}$.
Now use one more copy of  $f^{\otimes 2}$.
Suppose $f^{\otimes 2}(x_1, \ldots, x_s, y_1,  \ldots, y_s)
= f(x_1, \ldots, x_s) f(y_1,  \ldots, y_s)$, where $s$ is
the arity of $f$.
Replace the $(2k+1)$-th occurrence of $f$ in $\Omega_0$
by $f^{\otimes 2}$, using variables $y_1,  \ldots, y_s$ of  $f^{\otimes 2}$
to connect to the $s$ edges of the $(2k+1)$-th occurrence of $f$,
and leaving $x_1, \ldots, x_s$ as dangling edges.
This creates a $(\mathcal{F} \cup \{f^{\otimes 2}\})$-gate
with signature $c f$.
Hence
\[\operatorname{Holant}(\mathcal{F}, f)
\leq_{\rm T}^p
\operatorname{Holant}(\mathcal{F}, f^{\otimes 2}).\]
\end{proof}


Using Lemma~\ref{lm:Lin-Wang}, we can state the
following  dichotomy theorem from \cite{cailuxia-2017}
for  \#CSP$^2$.
\begin{theorem}\label{CSP2}
Let $\mathcal{F}$ be any set of complex-valued signatures in Boolean variables. Then $\#\operatorname{CSP}^2(\mathcal{F})$
is $\#\operatorname{P}$-hard unless
$\mathcal{F}\subseteq\mathscr{A}$ or
$\mathcal{F}\subseteq\alpha\mathscr{A}$ or
$\mathcal{F}\subseteq\mathscr{P}$ or
$\mathcal{F}\subseteq\mathscr{L}$
  in which cases the problem is computable in polynomial time.
\end{theorem}


The six-vertex model is the special case of the eight-vertex model with $a=x=0$ in $M(f)$.

\begin{theorem}\cite{cai:fu:xia}\label{dichotomy-six-vertex}
Let $f$ be a 4-ary signature with the signature matrix
$M(f)=\left[\begin{smallmatrix}
0 & 0 & 0 & b\\
0 & c & d & 0\\
0 & w & z & 0\\
y & 0 & 0 & 0
\end{smallmatrix}\right]$, the six-vertex model
$\operatorname{Holant}(\neq_2\mid f)$ is $\#\operatorname{P}$-hard except for the following cases:
 $f\in\mathscr{P}$, or
 $f\in\mathscr{A}$, or
 there is a zero in each pair $(b, y), (c, z), (d, w)$,
in which cases $\operatorname{Holant}(\neq_2\mid f)$ is computable in polynomial time.
\end{theorem}

\begin{definition}\label{redu-defi}
 A 4-ary signature $f$ is redundant iff in its  4 by 4 signature matrix
  the middle two rows are identical and the
 middle two columns are identical.
 We call $\left[\begin{smallmatrix}
f_{0000} & f_{0010} & f_{0011}\\
f_{0100} & f_{0110} & f_{0111}\\
f_{1100} & f_{1110} & f_{1111}
\end{smallmatrix}\right]$ the compressed signature matrix  of $f$.
 \end{definition}
\begin{theorem}\cite{caiguowilliams13}\label{redundant}
If $f$ is a redundant signature and its compressed signature matrix has full rank,
 then $\operatorname{Holant}(\neq_2|f)$ is \#$\operatorname{P}$-hard.
\end{theorem}







\subsection{M\"{o}bius Transformation}
A M\"{o}bius transformation~\cite{ahlfors} is
a mapping of the form ${\mathfrak z}
\mapsto \frac{a\mathfrak z+b}{c\mathfrak z+d}$,
where $\det \left[\begin{smallmatrix}
a & b \\
c & d
\end{smallmatrix}\right] \not =0$.
It is a bijective
 conformal map of the extended complex plane $\widehat{\mathbb{C}}
= \mathbb{C} \cup \{ \infty \}$ to itself.
%where the coefficients $a, b, c, d$ are complex numbers satisfying $ad-bc\neq 0$.
%A M\"{o}bius transformation is a bijective conformal function from the extended complex plane to the extended complex plane.
%It is a  conformal map that maps a circle to a circle or a line.
%In particular,
A M\"{o}bius transformation maps the unit circle $S^1=\{z \mid |z|=1\}$ to itself iff it is of the form
$\varphi(\mathfrak z)=e^{i\theta}\frac{\mathfrak{z}+\lambda}{1+\bar{\lambda} \mathfrak{z}}$ denoted by $\mathcal{M}(\lambda, e^{i\theta})$, where $|\lambda|\neq 1$. When $|\lambda|< 1$, it maps the interior of $S^1$ to the interior,
and when $|\lambda|> 1$, it maps the interior of $S^1$ to the exterior.
A M\"{o}bius transformation is determined by its values on any 3
distinct points. In particular if there are  5 distinct
points $\mathfrak{z}_i \in S^1$, such that $|\varphi({\mathfrak z}_i)|$
is either 0 or 1 or $\infty$, then it must map $S^1$ to $S^1$ in
a bijection.





==> 3outline-s.tex <==
\section{Main Theorem and Proof Outline}
\begin{theorem}\label{main:theorem}
Let $f$ be a 4-ary signature with the signature matrix
$M(f)=\left[\begin{smallmatrix}
a & 0 & 0 & b\\
0 & c & d & 0\\
0 & w & z & 0\\
y & 0 & 0 & x
\end{smallmatrix}\right]$.
If  $ax=0$, then  $\operatorname{Holant}(\neq_2|f)$ is
equivalent to the six-vertex model $\operatorname{Holant}(\neq_2|f')$
where $f'$ is obtained from $f$ by setting $a=x=0$,  i.e.,
$M(f')=\left[\begin{smallmatrix}
0 & 0 & 0 & b\\
0 & c & d & 0\\
0 & w & z & 0\\
y & 0 & 0 & 0
\end{smallmatrix}\right]$. Explicitly,
$\operatorname{Holant}(\neq_2|f)$
is $\#\operatorname{P}$-hard except in the following cases:
\begin{itemize}
\item $f'\in\mathscr{P}$,
\item $f'\in\mathscr{A}$,
\item there is at least one zero in each pair $(b, y), (c, z), (d, w)$.
\end{itemize}
If $ax\neq 0$, then $\operatorname{Holant}(\neq_2|f)$
is $\#\operatorname{P}$-hard except in the following cases:
\begin{itemize}
\item $f$ is $\mathscr{P}$-transformable;
\item $f$ is $\mathscr{A}$-transformable;
\item $f$ is $\mathscr{L}$-transformable.
\end{itemize}
In all listed cases, $\operatorname{Holant}(\neq_2|f)$ is computable in polynomial time.
\end{theorem}%%end of theorem

For any given $f$ in the eight-vertex model and any signature grid $\Omega$
with 4-regular graph $G$,
 any valid orientation
on $G$
for  Holant$_{\Omega}(\neq_2|f)$
must have an equal number of sources and sinks.
Hence the value  Holant$_{\Omega}(\neq_2|f)$
as a polynomial in $a$ and $x$ is in fact a polynomial in the product
$ax$.
So we can replace $(a,x)$ by any $(\tilde{a}, \tilde{x})$
such that $\tilde{a}\tilde{x} = ax$.
In particular,
let $\tilde{f}$  be a 4-ary signature with signature matrix
$M(\tilde{f})=\left[\begin{smallmatrix}
\tilde{a} & 0 & 0 & b\\
0 & c & d & 0\\
0 & w & z & 0\\
y & 0 & 0 & \tilde{a}
\end{smallmatrix}\right]$ where $\tilde{a}=\sqrt{ax}$,
then
Holant$_{\Omega}(\neq_2|f)=$Holant$_{\Omega}(\neq_2|\tilde{f})$.
Note that one can also switch the sign of both entries $(a,x)$.
If $a=0$,
  this is the six-vertex model and has been solved in Theorem~\ref{dichotomy-six-vertex} \cite{cai:fu:xia}.
In the following we assume $a=x\neq 0$.

Let $\textsf{N}$ be the number of zeros in $\{b, c, d, y, z, w\}$.
We define Case \uppercase\expandafter{\romannumeral1} to be
 $\textsf{N}\geq 1$
and there is at most one pair in $\{(b, y), (c, z), (d, w)\}$
that is $(0, 0)$.
We define Case \uppercase\expandafter{\romannumeral2} to be there are
(at least) two
 pairs in $\{(b, y), (c, z), (d, w)\}$ that are $(0, 0)$.
 Note that Case \uppercase\expandafter{\romannumeral1}
and Case \uppercase\expandafter{\romannumeral2} cover all cases that $\textsf{N}\neq 0$.
Finally we define Case \uppercase\expandafter{\romannumeral3} to be $\textsf{N}=0$.
Formally,
The three cases are defined as follows:
\begin{description}
\item {Case \uppercase\expandafter{\romannumeral1}:}
%There is are least one zero in $\{b, c, d, y, z, w\}$
$\textsf{N} \ge 1$ and there is at most one pair in
$\{(b, y), (c, z), (d, w)\}$ that is $(0, 0)$.

In this case we prove that Holant$(\neq_2|f)$ is \#P-hard.
We prove this by constructing a 4-ary signature $g$
in the six-vertex model, such that Holant$(\neq_2|g)$ is \#P-hard
by Theorem~\ref{dichotomy-six-vertex}, and prove that  Holant$(\neq_2|g)
\leq_T^p $ Holant$(\neq_2|f)$.
\item {Case \uppercase\expandafter{\romannumeral2}:}
There are (at least) two pairs in
$\{(b, y), (c, z), (d, w)\}$ that are $(0, 0)$.

By the symmetry of these three pairs (the group action of $S_3$ induced by $S_4$),
 we assume that $b=y=d=w=0$.
%%%%%%%%%%%%%%%%%%%%%
As $a \not =0$ we can normalize it to $a =1$.
We define a binary signature $g$ with the matrix
 $M(g) =
\left[\begin{smallmatrix}
1 & c \\
z & 1
\end{smallmatrix}\right]$.
We will reduce  \#CSP$^2(g)$ to
Holant$(\neq_2|f)$.
This will be accomplished by replacing every variable
in an instance $\Omega$ of  \#CSP$^2(g)$
by a cycle of even length,
such that there is a 1-1 correspondence between assignments
in $\Omega$ and valid configurations of the eight-vertex model
Holant$(\neq_2|f)$, that preserves the product of the weights.

%%%%%%%%%%%%%%%%%%%%
%We can define a set of circuits, and
%define a \#CSP problem where the variables correspond to
%the circuits, and the valid assignments in the eight-vertex model
%Holant$(\neq_2|f)$ ensure that there are exactly two valid
%configurations on these circuits that correspond to
%the two cyclic orientations.
%We further show that this is in fact a \#CSP$^2$ problem, where
%each variable appears an even number of times.  This is because
%the support structure of $f$ ensures that these circuits all have even
%length.
%
%Then we reduce \#CSP$^2(g)$ to
%Holant$(\neq_2|f)$,
%%, where $g$ is a binary signature whose entries come from the
%%support of $f$.
%where $g$ is a binary signature
%with matrix $M(g) =
%\left[\begin{smallmatrix}
%a & c \\
%z & a
%\end{smallmatrix}\right]$.
%%=(a, c, z, a)^T$.
%%Note that in \cite{cai:fu:xia}, the connection is between Holant and \#CSP.
%%\#CSP$^2$ is necessary for this paper since if the evaluation of Holant$(\neq_2|f)$ is not zero,
%%then the number of vertices in each circuit has to be even.

By Theorem~\ref{CSP2}, if $g\notin\mathscr{P}\cup\mathscr{A}\cup\alpha\mathscr{A}\cup\mathscr{L}$,
then \#CSP$^2(g)$ is \#P-hard. In this case Holant$(\neq_2|f)$ is \#P-hard.
If $g\in\mathscr{P}\cup\mathscr{A}\cup\alpha\mathscr{A}\cup\mathscr{L}$,
we show that $f$ is $\mathscr{P}$-transformable or $\mathscr{A}$-transformable.
Thus  Holant$(\neq_2|f)$ is tractable.
\item {Case \uppercase\expandafter{\romannumeral3}:}
$\textsf{N}=0$, i.e., all values in $\{b, c, d, y, z, w\}$ are nonzero.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%555%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this case we prove that  Holant$(\neq_2|f)$ is tractable
in the listed cases, and  \#P-hard otherwise.
The main challenge here is when we prove \#P-hardness for some
signatures $f$, the interpolation needs certain quantities
not to repeat after iterations. If we can only produce a root of unity, then its powers will
repeat after only a bounded number of steps in an iteration.
Typically one satisfies such a requirement
by producing quantities of complex norm not equal to 1.
   But for some $f$,
    provably the only such quantities
that can be produced are all of complex norm 1.

Our main new idea is to use M\"{o}bius transformations.
But before getting to that, there are some settings where we cannot do so, either because we don't
have the initial signature to start the process, or the matrix that
would define the M\"{o}bius transformation is singular.
   So we first treat the following two special cases.
      \begin{itemize}
      \item If $b=\epsilon y$, $c=\epsilon z$ and $d=\epsilon w$, where $\epsilon = \pm 1$, by a rotational symmetric gadget,
      we get some redundant signatures (Definition~\ref{redu-defi}).
 If one of the compressed matrices of these redundant signatures has full rank,
      then we can prove \#P-hardness.
      If all of these compressed matrices are degenerate, then we get a system of equations of $\{a, b, c, d\}$.
      To satisfy these equations,  $f$ has a very special form.
      Then we show that either
$f$ is $\mathscr{A}$-transformable or we can construct
an arity 4 signature
$g = \left[\begin{smallmatrix}
t & 0 & 0 & 1\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
1 & 0 & 0 & \frac{1}{t}
   \end{smallmatrix}
      \right]$, which is actually
 a symmetric signature $g = [g_0, g_1, g_2, g_3, g_4]
=[t, 0, 1, 0, \frac{1}{t}]$, with $t\neq 0$.
Here $g_w$ is the value of $g$ on all inputs of Hamming weight $w$.
      By a holographic transformation using $T=\left[
   \begin{smallmatrix}
   1 & t\\
   \frak{i} & -\frak{i}t
   \end{smallmatrix}
      \right]
=\sqrt{2} Z 
\left[
   \begin{smallmatrix}
   1 & 0\\
   0 & t
   \end{smallmatrix}
      \right]
=\left[
   \begin{smallmatrix}
   1 & 1\\
   \frak{i} & -\frak{i}
   \end{smallmatrix}
      \right]
\left[
   \begin{smallmatrix}
   1 & 0\\
   0 & t
   \end{smallmatrix}
      \right]
=\left[
   \begin{smallmatrix}
   1 & 0\\
   0 & \frak{i}
   \end{smallmatrix}
      \right]
\left[
   \begin{smallmatrix}
   1 & 1\\
   1 & -1
   \end{smallmatrix}
      \right]
\left[
   \begin{smallmatrix}
   1 & 0\\
   0 & t
   \end{smallmatrix}
      \right]
$ on
Holant$(\neq_2|f, g)$,
because $(=_2)Z^{\otimes 2} = (\neq_2)$ and therefore
$(\neq_2)(T^{-1})^{\otimes 2} = \frac{1}{2t} (=_2)$,
the signature 
$(\neq_2)$ is transformed to $(=_2)$ on the LHS up to a nonzero scalar.
Similarly $g$ is
% $[t, 0, 1, 0, \frac{1}{t}]$ is
 transformed to $T^{\otimes 4} g$ on the RHS,
which is $(=_4)$ up to a nonzero scalar.
 Therefore we have the equivalence
      Holant$(\neq_2|f, g)\equiv^p_T$ \#CSP$^2(T^{\otimes 4}f)$.
      This implies that
       Holant$(\neq_2 \mid f)$ is either \#P-hard, or
      $f$ is $\mathscr{P}$-transformable, or $\mathscr{A}$-transformable, or $\mathscr{L}$-transformable
      by Theorem~\ref{CSP2}.
         \item If $by=cz=dw$,
then either we can realize a non-singular redundant signature or $f$ is
$\mathscr{A}$-transformable.
    \end{itemize}
      If $f$ does not belong to the above two cases,
      by the symmetry of the pairs $\{(b, y), (c, z), (d, w)\}$, we may assume that
      $cz\neq dw$, i.e., the inner matrix
$\left[
   \begin{smallmatrix}
   c & d\\
   w & z
   \end{smallmatrix}
      \right]$
of $M(f)$ has full rank.
      Then
      we
want to realize
binary signatures of the form $(0, 1, t, 0)^T$,
      for arbitrary values of $t$. If this can be done,
      by carefully choosing the values of $t$,
      we will prove \#P-hardness by
      \begin{itemize}
      \item constructing a signature that belongs to Case \uppercase\expandafter{\romannumeral1}
      (Case A in the proof of Lemma~\ref{with-any-binary}), or
      \item constructing a redundant signature whose compressed signature matrix has full rank
      (Case B in the proof of Lemma~\ref{with-any-binary}), or
      \item
      constructing the symmetric signature $[1, 0, -1, 0, 1]$ by gadget construction. Then by
       the holographic transformation using
 $T=\left[
   \begin{smallmatrix}
   1 & \frak i\\
   \frak{i} & 1
   \end{smallmatrix}
      \right]
=
\left[
   \begin{smallmatrix}
1 & 0\\
0 & \frak{i}
   \end{smallmatrix}
      \right]
\left[
   \begin{smallmatrix}
1 & 1\\
1 & -1
\end{smallmatrix}
      \right]
\left[
   \begin{smallmatrix}
1 & 0\\
0 & \frak{i}
   \end{smallmatrix}
      \right]
$, we have
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%here
      \begin{center}
      Holant$(\neq_2|f, [1, 0, -1, 0, 1], (0, 1, t, 0)^T)\equiv^p_T$ \#CSP$^2(T^{\otimes 4}f, T^{\otimes 2}(0, 1, t, 0)^T))$,
      \end{center}
because $(\ne_2) (T^{-1})^{\otimes 2}$ is $(=_2)$,
and $T^{\otimes 4} [1, 0, -1, 0, 1]$ is $(=_4)$, both up to  a nonzero scalar.
      Then we can prove \#P-hardness  by Theorem~\ref{CSP2}
      (Case C in the proof of Lemma~\ref{with-any-binary}).
      \end{itemize}
      %Follows from the result of Case \Rmnum{3},
      %we get the \#P-hardness result.


\vspace{.1in}

      We realize binary signatures by connecting $f$ with $(\neq_2)$.
This corresponds naturally to a M\"{o}bius transformation.
      By discussing the following different forms of binary signatures we get,
      we can either realize arbitrary $(0, 1, t, 0)^T$, then  Holant$(\neq_2|f)$
      is \#P-hard, or $f$ is $\mathscr{A}$-transformable under some nontrivial holographic transformation.
\begin{itemize}
         \item If we can get a signature of the form $g = (0, 1, t, 0)^T$ where $t\neq0$ is not a root of unity, then by connecting a chain of $g$, we can
get polynomially many distinct binary signatures $g_i=(0, 1, t^i, 0)^T$.
         Then, by interpolation, we can realize
 arbitrary binary signatures of the form $(0, 1, s, 0)^T$.

         \item Suppose we can get a signature of the form $(0, 1, t, 0)^T$, where $t\neq0$ is an $n$-th primitive root of unity $(n\geq 5)$. Now, we only have $n$ many different signatures $g_i=(0, 1, t^i, 0)^T$.
         But we can relate $f$ to a M\"{o}bius transformation
$\varphi(\mathfrak{z}): \mathfrak{z} \mapsto
\dfrac{c \mathfrak{z} + d}{w \mathfrak{z} + z}$,
%%%%%%%%%%%%{{{{{{{{{{{{
due to
$\det\left[\begin{smallmatrix}
c & d\\
w & z 
\end{smallmatrix}\right] \not =0$.
%$ax-cz \neq 0$ and $by-cz \neq 0$.
         For the M\"{o}bius transformation $\varphi$, we can realize the signatures $g= (0, 1, \varphi(t^i), 0)^T$.
If $|\varphi(t^i)|\neq 0, 1$ or $\infty$ for some $i$,
then this is treated above.
Otherwise, since $\varphi$ is a bijection on the extended complex plane
$\widehat{\mathbb{C}}$, it can map at most two points of  $S^1$ to
$0$ or $\infty$.
         Hence, $|\varphi(t^i)|= 1$ for at least three $t^i$.
But a M\"{o}bius transformation is determined by any three distinct points.
This implies that $\varphi$  maps  $S^1$ to itself.
 Such M\"{o}bius transformations  have a known special form
$e^{i\theta}\dfrac{\mathfrak{z}+\lambda}{1+\bar{\lambda}\mathfrak{z}}$.
By exploiting its property we can construct a signature $f'$ such that
its corresponding M\"{o}bius transformation $\varphi'$
%infinite projective order.
defines an infinite group. This implies
that $\varphi'^k(t)$ are all distinct. Then, we can get polynomially
 many distinct binary signatures $(0, 1, \varphi'^k(t), 0)$, and
realize arbitrary binary signatures of the form $(0, 1, s, 0)^T$ (Lemma~\ref{non:root:of:unity}).

         \item Suppose we can get a signature of the form $(0, 1, t, 0)^T$ where $t\neq0$ is an $n$-th primitive root of unity $(n=3, 4)$. Then we can either relate it to two M\"{o}bius transformations mapping the unit circle to itself, or
realize the $(+, -)$-pinning $(0, 1, 0, 0)^T = (1,0) \otimes (0,1)$.
\item Suppose we can get $(0, 1, 0, 0)^T$.
 By connecting $f$ with it, we can get new signatures of the form $(0, 1, t, 0)^T$. Similarly, by analyzing the value of $t$,
         we can either realize arbitrary binary signatures of the form $(0, 1, s, 0)^T$, or a redundant signature
         whose compressed signature matrix has full rank, or a signature in Case \uppercase\expandafter{\romannumeral1}, which is \#P-hard,
          or we prove that $f$ is $\mathscr{A}$-transformable under a
 holographic transformation
%such as
          $\left[\begin{smallmatrix}
1 & 0 \\
0 & \gamma
\end{smallmatrix}\right]$, where $\gamma^2= \alpha$  or $ \gamma^2= \frak{i}$
(Theorem~\ref{with:(0,1,0,0)}).
         \item Suppose we can only get signatures of the form $(0, 1, \pm 1, 0)^{T}$. That implies $a=\epsilon x$, $b=\epsilon y$ and $c=\epsilon z$, where $\epsilon=\pm 1$.  This has been treated before.
    \end{itemize}
\end{description}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%beginning of mobious


    %\item[\Rmnum{4}.]\label{case4} %More than three zeros or
    %There is exactly one zero in each pair. %\plholant{\neq_2}{f} is tractable since \holant{\neq_2}{f} is tractable
    %All are tractable since in this case, $\holant{\neq_2}{f}$ is tractable \cite{}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of mobious





%%%%%%%%%%%%%%%%%%%%%%%%%%%5argument that we can not get any binary signature except for (0, 1, 1, 0) if b=y, c=z, d=w
%Let $f$ a 4-ary signature whose signature matrix is
%$M(f)=\left[\begin{smallmatrix}
% 0 & 0 & 0 & a\\
% 0 & b & c & 0\\
% 0 & \epsilon c & \epsilon & 0\\
% \epsilon z & 0 & 0 & 0\\
%\end{smallmatrix}\right]$ where $\epsilon=\pm 1$.
%Given $n$ copies of $f$, leaving two edges as dangling edges, and connecting other edges of these copies using $\neq_2$, we get a gadget
%$\Gamma(x_1, x_2, \cdots, x_m; y_1, y_2)$
%whose signature $g(y_1, y_2)$ is a binary signature, where the variables
%$x_1, x_2, \cdots, x_m$ correspond to the internal edges of $\Gamma$ and $y_1, y_2$ correspond to
%the dangling edges of $\Gamma$. Thus $g(y_1, y_2)=\displaystyle\sum_{x_1, x_2, \cdots, x_m\in\{0, 1\}}H(x_1, x_2, \cdots, x_m; y_1, y_2)$, where
%$H(x_1, x_2, \cdots, x_m; y_1, y_2)$
%is the value of the signature grid on an assignment of all edges in $\Gamma$, which is the product of
%evaluations at all vertices in  $\Gamma$.
%Note that $f$ satisfies even parity constraint and $\neq_2$ satisfies odd parity constraint.
%Thus $g$ has to satisfy parity constraint.
%Note there are $2n-1$ copies of $\neq_2$ in $\Gamma$. This implies that $g$ has to satisfy odd parity constraint, i.e.,
%$g(0, 0)=g(1, 1)=0$.
%Moreover, $H(x_1, x_2, \cdots, x_m; 0, 1)\neq 0$ iff $H(\bar{x_1}, \bar{x_2}, \cdots, \bar{x_m}; 1, 0)\neq 0$
%and $H(x_1, x_2, \cdots, x_m; 0, 1)=\epsilon^nH(\bar{x_1}, \bar{x_2}, \cdots, \bar{x_m}; 1, 0)$.
%Thus $g(0, 1)=\epsilon^n g(1, 0)$.
%This implies that we can not construct any binary signature except for $(0, 1, \epsilon, 0)^T$ in this case.%

 %In any instance of Holant$_{\Omega}(\neq_2|f)$ on the bipartite graph
%$G=(V_1, V_2, E)$, since the signatures labelled on the vertices on
%left side is $\neq_2$, thus the number of the edges that are assigned 0 is equal to the number of the edges that
%are assigned 1 in any assignments which give nonzero evaluation.
%Thus Holant$_{\Omega}(\neq_2|f)$ can be expressed as a polynomial $\sum_{i=0}^{\lfloor\frac{|V_2|}{2}\rfloor} c_ia^ix^i$.
%So if we replace $(a, x)$ by $(\sqrt{ax}, \sqrt{ax})$, Holant$_{\Omega}(\neq_2|f)$ will not change.
%This implies that we may assume that $a=x$.%
%
%
%
%If there are two of $(b, y), (c, z), (d, w)$ are $(0, 0)$, without loss of generality we assume that
% $(c, z)=(d, w)=(0, 0)$, then by a global simulation, we have
%Holant$(\neq_2|f)\geq_{T}$\#CSP$^2(g)$, where $g=(a, b, y, x)$ is a binary signature.
%It is obvious that if \#CSP$^2(g)$ is \#P-hard, then Holant$(\neq_2|f)$ is \#P-hard.
%We finish the proof of this case by proving that if \#CSP$^2(g)$ is tractable, then Holant$(\neq_2|f)$ is tractable.%
%
%If there is at least one of $b, y, c, z, d, w$ is zero and there is at most one of $(b, y), (c, z), (d, w)$ is $(0, 0)$,
%Holant$(\neq_2|f)$ is \#P-hard. In these cases, we always
%finish the proof by reducing to
% a six-vertex problem which is \#P-hard by gadget construction.
%
% Now we can assume that $bcdyzw\neq 0$.
 %Then we consider two special cases.
% The first is $b=\epsilon y, c=\epsilon z, d=\epsilon w$, where $\epsilon=\pm 1$. In this case, we can not construct any binary signatures
% except for $(0, 1, \pm 1, 0)^T$. So we can not simplify $f$ by binary signatures.
% We use a cross gadget to get some 4-ary rotational symmetric signatures that are redundant signatures.
% So if the compressed signatures of them has full rank, then we can prove hardness.
% Otherwise, Holant$(\neq_2|f)$ is tractable or $f$ has a very special form. Then we can prove hardness by the dichotomy theorem of six-vertex problems.%
%
 %Another special case is $by=cz=dw$. In this case, for any permutation $(i, j, k, l)$ of $(1, 2, 3, 4)$, the inner matrix of
 %$M_{x_ix_j, x_kx_l}(f)$ is degenerate. We prove hardness by constructing a redundant signature whose compressed signature has full rank,
 %or by constructing the symmetric signature $[t, 0, 1, 0, \frac{1}{t}]$, after a holographic transformation, the Holant problem can be reduced to
 %\#CSP$^2$ problems.%
%
% After these two cases, we can assume that the inner matrix of the signature matrix  of $f$ has full rank and
% we have a binary signature $(0, 1, t, 0)^T$, where $t^2\neq 0, 1$.
%  If $t$ is not a root of unity, then we can get $(0, 1, u, 0)^T$ for any
%$u\in\mathbb{C}$ by interpolation. But if $t$ is a root of unity indeed, except for some tractable cases, we still can get $(0, 1, u, 0)^T$ for any
%$u\in\mathbb{C}$. This is a new technique.
%Using these binary signatures, we can simplify the form of $f$ greatly, then we can finish the proof.%
%%
%\begin{lemma}\label{affine-support}
%If the support of $f$ is not affine, then hard.
%\end{lemma}
%Now $M(f)=\left[\begin{smallmatrix}
%a & 0 & 0 & b\\
%0 & c & d & 0\\
%0 & w & z & 0\\
%%y & 0 & 0 & a
%%\end{smallmatrix}\right]$ with $a\neq 0$.


==> 4spin-s.tex <==
\section{Two Inner Pairs Are $(0, 0)$}
If there are two inner pairs that are $(0, 0)$, by the symmetry
of the three inner pairs $(b, y), (c, z), (d, w)$, we may assume that $b=y=d=w=0$.
Then we have the following lemma.
\begin{lemma}\label{spin}
Let $f$ be a 4-ary signature with the signature matrix $M(f)=\left[\begin{smallmatrix}
 a & 0 & 0 & 0\\
 0 & c & 0 & 0\\
 0 & 0 & z & 0\\
 0 & 0 & 0 & a\\
\end{smallmatrix}\right],$
%\begin{center}
%\begin{equation}\label{one-zero-pair-matrix-form}
%M_{x_sx_t, x_ux_v}(f)=\begin{bmatrix}
%\alpha & 0 & 0 & 0\\
%0 & \beta & 0 & 0\\
%0 & 0 & \gamma & 0\\
%0 & 0 & 0 & \delta\\
%\end{bmatrix},
%\end{equation}
%\end{center}
%where $\{s,t,u,v\}$ is a permutation of $\{1, 2, 3, 4\}$.
 then $\operatorname{Holant}(\neq_2\mid f)$
is \#$\operatorname{P}$-hard unless
$f$ is $\mathscr{A}$-transformable, or
$f\in\mathscr{P}$,
  in which case the problem is computable in polynomial time.
\end{lemma}
\begin{proof}
Tractability follows from Theorem~\ref{CSP2}.

As $a \not =0$ we can normalize it to $a=1$.
Let $g(x_1, x_2)$ be the binary signature
  $M(g) = \left[\begin{smallmatrix}
 1 & c \\
 z & 1
\end{smallmatrix}\right]$
in matrix form.
%(not necessarily symmetric)
This means that
$g_{00} = g_{11} = 1 = f_{0000}=f_{1111}$, $g_{01} =c = f_{0101}$
and $g_{10} =z = f_{1010}$.
%In matrix form $g(x, y)$ is given by
We prove that
$\operatorname{\#CSP}^2(g)\leq^p_{\operatorname{T}}\operatorname{Holant}(\neq_2\mid f)$
in two steps.
In each step, we begin with a signature grid and end with a new signature grid such that the Holant values of both signature grids are the same.

For step one, let $G=(U, V, E)$ be a bipartite graph
representing  an instance of \#CSP$^2(g)$, where each $u \in U$ is a variable,
and each $v \in V$ has degree two and is labeled $g$.
%Suppose $g(u, u')$ is applied to the variables $u$ and $u'$.
For every vertex $u \in U$,
we define a cyclic order of the edges incident to $u$,
 and decompose $u$ into $2k = \deg(u)$ vertices.
 Then we connect the $2k$
edges originally incident to $u$ to these $2k$ new vertices
so that each vertex is incident to exactly one edge.
We also connect these $2k$ new
 vertices in a cycle according to the cyclic order.
%(see Figure~1 (b) in the Appendix).
Thus, in effect we have replaced $u$ by a cycle of length $2k = \deg(u)$.
% by their incident edges.
    Each of  $2k$ vertices has degree 3, and we assign them $(=_3)$.
Clearly this does not change the value of the partition function. The resulting graph has the following properties: (1) every vertex has either degree 2 or degree 3; (2) each degree 2 vertex is connected
to degree 3 vertices;
%%% i avoid talking about two degree 3 vertices because they could be the same.
(3) each degree 3 vertex is connected to exactly one degree 2 vertex.
% i avoid talking about two other degree 3 vertices because they may not
% distinct "other".
%%%%%%%%%%%%%%%%%%%%%%%%%%%%special cases:
% if u has deg 2, then the cycle is 2 parallel edges
% if u has deg 1, the cycle is a loop. (eventually all "cycles" edges will
% be given \neq
% if g has two identical varaibles as input, then the "two cycles" that
% g connect to is the same cycle.
% if var=0 <--> + <--> counterclockwise order on cycle
%    var=1 <--> - <--> clockwise order on cycle
% take g as vetical line segment top is 1st var, bottom is 2nd var
% say counterclockwise on cycle <--> is 0 when enter external-cycle-vertex
%                                    and 1 when leave external-cycle-vertex
%              when traveling in counterclockwise
% similarly,
%            clockwise on cycle <--> is 0 when enter external-cycle-vertex
%                                    and 1 when leave external-cycle-vertex
%              when traveling in clockwise
% THEN when placing f after contraction, x_1 on NW, x_2 on NE
%                                        x_3 on SW, x_4 on SE
% then e.g., if input to g is 00, then
% x_1 =0, x_4 =0  This gives entry \alpha f_{0 1 1 0}
%            if input to g is 01, then
% x_1 =0, x_4 =1  This gives entry \alpha f_{0 1 0 1}
%            if input to g is 10, then
% x_1 =1, x_4 =0  This gives entry \alpha f_{1 0 1 0}
%            if input to g is 11, then
% x_1 =1, x_4 =1  This gives entry \alpha f_{1 0 0 1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% if g has two neighbors as the same vertex x, x
% the two edges from x to g counts as two distinct edges and become two
% verteices on the cycle.  when contracting, these two become the same vertex.
% say the cycle x has become has the top horizontal edge with 2 external
% corners for g.  on top of that edge there is g-edge
% contract g --> the top edge becomes a loop (with \neq)
%from R to L, 4 bits as half edges along the top edge, label them
% x1, x_2, x_4, x_3.
% if x=0, counterclock,
%it's 0 (enter external corner) 1 (top edge= \neq) 0 (enter 2nd external corner)1 so x_1=x_4=0.
% if x=1, clock,  still enumerate from R to L:
%it's 1 (enter external corner) 0 (top edge= \neq) 1 (enter 2nd external corner) 0 so x_1=x_4=1.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now step two.
We add a vertex on every edge of each cycle  $C_u$
of length $2k =  \deg(u)$, making $C_u$ a cycle of length $4k$.
(This is shown in Figure~\ref{holant-csp-b}).
Name the vertices $1 ,2, \ldots, 4k$ in cyclic order,
with the newly added vertices numbered $1,3, \ldots, 4k-1$. There are
$k$ pairs of these odd numbered vertices
$(1,3), (5,7), \ldots, (4k-3, 4k-1)$.
We will merge each pair $(4i-3, 4i-1)$ ($1 \le i \le k$)
to form a new vertex of degree 4,
and assign a signature $f$ on it.
(This ``pinching'' operation is illustrated by the dotted line
in Figure~\ref{holant-csp-b}). The input variables of $f$
are carefully assigned so that the two incoming edges originally
at $4i-3$ are named $x_1$ and $x_3$,
and the other two incoming edges originally
at $4i-1$  are named $x_2$ and $x_4$.
Note that the support of $f$ ensures that the values
at $x_1$ and $x_3$ are equal, and
the values $x_2$ and $x_4$ are equal.
For every even numbered vertex $2i$ ($1 \le i \le 2k$) on $C_u$,
it is currently connected to a vertex $v$ of degree 2 labeled $g$.
Suppose in the  instance of \#CSP$^2(g)$,
the constraint $g(u, u')$ is applied to the variables $u$ and $u'$,
in that order.
Then the other adjacent vertex of $v$ is some  even numbered vertex  $2j$
 on the cycle $C_{u'}$ for the variable $u'$.
We will contract the two incident edges at $v$,
merging the vertices  $2i$ on $C_u$ and  $2j$ on $C_{u'}$,
to form a new vertex $v'$ of degree 4, and assign a copy of $f$ on it.
The input variables of $f$
are carefully assigned so that the two incoming edges originally
at $2i$ of $C_u$ are named $x_1$ and $x_3$,
and the other two incoming edges originally
at $2j$  of $C_{u'}$ are named $x_2$ and $x_4$.
The support of $f$ ensures that the values of
 $x_1$ and $x_3$ are equal and the values of
 $x_2$ and $x_4$ are equal.
(This  is illustrated in Figure~\ref{holant-csp-c}).
Finally  we put a $(\ne_2)$ on every edge.
This completes the definition of an instance of
 $\operatorname{Holant}(\neq_2\mid f)$ in this
reduction.

Note that if we traverse the cycle $C_u$, by the support of
$f$ and the $(\ne_2)$ on every edge, there exists some $\epsilon =0, 1$,
such that all four edges for
the  $f$ at any odd numbered pair $(4i-3, 4i-1)$
must take the same value $\epsilon$, and the two adjacent edges
at every even numbered vertex $2i$ must take the same value $1-\epsilon$.
Therefore there is a 1-1 correspondence between
0-1 assignments for the variables in  \#CSP$^2(g)$
and valid configurations in $\operatorname{Holant}(\neq_2\mid f)$.
Furthermore, at every odd numbered pair $(4i-3, 4i-1)$
the value is $f_{0000}=1$ or $f_{1111}=1$.
The value of $f$ at the vertex $v'$ formed by contraction at $v$
reflects perfectly the value of $g(u,u')$.
Hence,
$\operatorname{\#CSP}^2(g)\leq^p_{\operatorname{T}}\operatorname{Holant}(\neq_2\mid f)$.


%Next we determine what is the signature on $v'\in V'$ after this contraction. Clearly there are only two inputs to each original cycle due to the $(\neq_2)$ on it. Therefore its support is $\{0110, 0101, 1010, 1001\}$. Moreover, the weight on $0110$ is $\alpha$,  the weight on $0101$ is $\beta$, the weight on $1010$ is $\gamma$, and the weight on $1001$ is $\delta$. Hence it is exactly the signature $f$. So we have
%$\operatorname{\#CSP}(g)\leq _{\operatorname{T}}
%\operatorname{Holant}(\neq_2\mid f).$
%

If $g\notin\mathscr{P}\cup\mathscr{A}\cup\alpha\mathscr{A}\cup\mathscr{L}$, then
$\operatorname{\#CSP}^2(g)$ is $\#$P-hard by Theorem~\ref{CSP2}.
It follows that $\operatorname{Holant}(\neq_2\mid  f)$ is \#P-hard.
Otherwise, note that $f(x_1,x_2,x_3,x_4)=g(x_1,x_2)\cdot \chi_{x_1 = x_3} \cdot \chi_{x_2 = x_4}$.
Hence, $g \in \mathscr{A} \cup \mathscr{P}$ implies $f \in \mathscr{A} \cup \mathscr{P}$.
Since $g_{00}\neq 0$, if $g\in\mathscr{L}$, then $g\in\mathscr{A}$
by the definition of $\mathscr{L}$, and
therefore $f \in\mathscr{A}$.
Finally,  if $g\in\alpha\mathscr{A}$, i.e., $\left[
\begin{smallmatrix}
1 & 0\\
0 & \alpha
\end{smallmatrix}
\right]^{\otimes 2}g=(1, \alpha c, \alpha z, {\frak i})^T\in \mathscr{A}$,
then after the holographic transformation to $f$ using $\left[\begin{smallmatrix}
1 & 0\\
0 & \beta
\end{smallmatrix}
\right]$, where $\beta^2=\alpha$, we get the signature $\widehat{f}$ whose signature matrix is
$\left[\begin{smallmatrix}
1 & 0 & 0 & 0\\
0 &  \alpha c & 0 & 0\\
0 & 0 &  \alpha z & 0\\
0 & 0 & 0 & {\frak i}\\
\end{smallmatrix}
\right]$, Since
 $\widehat{f}\in\mathscr{A}$,
$(\ne_2)\left[
\begin{smallmatrix}
1 & 0\\
0 & \beta
\end{smallmatrix}
\right]^{\otimes 2}
$ is $(\ne_2)$ up to a nonzero scalar, we conclude that
$f$ is $\mathscr{A}$-transformable.
This finishes the proof.
\end{proof}
\input{holantcsp-s}




==> 5mobi-s.tex <==
\section{Interpolation via M\"{o}bius Transformation}


%For a binary signature $(0, u, v, 0)$ with $uv\neq 0$, let $\rho=\frac{v}{u}$ for $u\neq 0$.
%When we connect $x_3$ and $x_4$ by the binary signature $(0, u, v, 0)$, we get a binary signature
%$(0, cv+du, wv+zu, 0)$.
%If $cv+du=0, wv+zu\neq 0$, then we get $(0, 0, 1, 0)$ after the scalar $wv+zu$.
%Otherwise, we get the binary signature $(0, 1, \rho', 0)$, where $\rho'=\frac{wv+zu}{cv+du}$.
%This shows that we get $(0, 1, \rho', 0)$ by $(0, 1, \rho, 0)$ iff $f(\rho)=\rho'$
%and we get $(0, 0, 1, 0)$ iff $f(\rho)=\infty$, where $f(\rho)=\frac{w\rho+z}{c\rho+d}$.

\begin{lemma}\label{non:root:of:unity}
Let $g=(0, 1, t, 0)^T$ be a binary signature where $t\neq 0$ and is not a root of unity,  then for any signature set
$\mathcal{F}$, and any $u\in\mathbb{C}$, we have
$\operatorname{Holant}(\neq_2 |\mathcal{F}, (0, 1, u, 0)^T)\leq^p_{\operatorname{T}}\operatorname{Holant}(\neq_2 |\mathcal{F}, g).$
\end{lemma}

Note that having $g=(0, 1, t, 0)^T$ is equivalent to having
$g'(x_1, x_2) = g(x_2, x_1) = (0, t, 1, 0)^T$.

\begin{lemma}\label{construct-binary}
Let $g=(0, 1, t, 0)^T$ be a binary signature where $t$ is an $n$-th primitive root of unity, $n\geq 5$,  and $f$
be a signature with the signature matrix
 $M(f)=\left[\begin{smallmatrix}
 a & 0 & 0 & b\\
 0 & c & d & 0\\
 0 & w & z & 0\\
 y & 0 & 0 & a\\
\end{smallmatrix}\right]$ with $abcdyzw\neq 0$, where
$\left[\begin{smallmatrix}
  c & d\\
  w & z
\end{smallmatrix}\right]$
has full rank, then for any $u\in\mathbb{C}$,
$\operatorname{Holant}(\neq_2 | f, (0, 1, u, 0)^T)\leq^p_{\operatorname{T}}\operatorname{Holant}(\neq_2 | f, g).$
\end{lemma}
\begin{proof}
By connecting two copies of $g$ using $(\neq_2)$, we get the signature $g_2$ whose signature matrix is
$
M(g_2)=
\left[\begin{smallmatrix}
 0& 1\\
 t& 0\\
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
 0& 1\\
 1& 0\\
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
 0& 1\\
 t& 0\\
\end{smallmatrix}\right]=
\left[\begin{smallmatrix}
 0& 1\\
 t^2& 0\\
\end{smallmatrix}\right]
.$
Similarly, we can construct  $g_i=(0, 1, t^i, 0)^T$ for $1\leq i\leq 5$.
 Since the order $n\geq 5$,
  $g_i$ are distinct pairwise for $1\leq i\leq 5$.



%{\bf This part has been moved to preliminary. }
%\{For any binary signature $g$ in the form of %$g^{(x_1, x_2)}=(0, a, b, 0)$, notice that %$g^{(x_2, x_1)}=(0, b, a, 0)$. Then we have
%\begin{align*}
%& M_{x_s x_t, x_v x_u}Ng^{(x_1, x_2)}\\
%=& M_{x_s  x_t, x_v x_u}
%\begin{bmatrix}
%0 & 0 & 0 & 1 \\
%0 & 0 & 1 & 0 \\
%0 & 1 & 0 & 0 \\
%1 & 0 & 0 & 0 \\
%\end{bmatrix}
%\begin{bmatrix}
%0\\
%a\\
%b\\
%0\\
%\end{bmatrix} \\
%= & M_{x_s x_t, x_v x_u}
%\begin{bmatrix}
%0\\
%b\\
%a\\
%0\\
%\end{bmatrix}\\
%= & M_{x_s  x_t, x_v x_u}g^{(x_2, x_1)}.
%\end{align*}
%That means connecting the variables $x_v$, $x_u$ of the signature $f$ with the variables $x_1$, $x_2$ of the signature $g$ using $(\neq_{2})$ are equivalent to connecting the variables $x_v$, $x_u$ of the signature $f$ with the variables $x_2$, $x_1$ of the signature $g$ directly. Since $g$ is a binary signature, we can rotate it by $180$ degree. Then the variables $x_1$ and $x_2$ change their positions with each other, and that rotation do not destroy the planar graph. \}



By connecting the variables $x_3$ and $x_4$ of the signature $f$ with the variables $x_1$ and $x_2$ of $g_i$ using $\neq_2$
for $1 \leq i \leq 5$ respectively,  we get binary signatures
$$h_i=M(f)Ng_i=
\left[\begin{smallmatrix}
a & 0& 0& b\\
0 & c& d& 0\\
0 & w& z& 0\\
y & 0 & 0 & a
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
0\\
t^i\\
1\\
0\\
\end{smallmatrix}\right]
=\left[\begin{smallmatrix}
0\\
ct^i+d\\
wt^i+z\\
0\\
\end{smallmatrix}\right].
$$
Let $\varphi(\mathfrak z)=\dfrac{c\mathfrak z+d}{w\mathfrak z+z}$.
Since $\det\left[\begin{smallmatrix}
c & d\\
w & z
\end{smallmatrix}\right]\neq 0$,
$\varphi(\mathfrak z)$ is a M\"{o}bius transformation  of the  extended  complex  plane $\widehat{\mathbb{C}}$.
We rewrite $h_i$ as $(wt^i+z)(0, \varphi(t^i), 1, 0)^T$, with the understanding that if $wt^i+z=0$, then $ \varphi(t^i)=\infty$, and we define
$(wt^i+z)(0, \varphi(t^i), 1, 0)^T$ to be $(0, ct^i+d, 0, 0)^T$.
Having $(0, \varphi(t^i), 1, 0)^T$ is equivalent to
having $(0, 1, \varphi(t^i), 0)^T$.
If there is a $t^i$ such that $\varphi(t^i)\neq 0, \infty$ or a root of unity for $1\leq i\leq 5$,
 then by Lemma~\ref{non:root:of:unity},
 $\operatorname{Holant}(\neq_2 | f, (0, 1, u, 0)^T)\leq^p_{\operatorname{T}}\operatorname{Holant}(\neq_2 | f, (0, 1, \varphi(t^i), 0)^T)$,
for all $u \in \mathbb{C}$.
 Otherwise, $\varphi(t^i)$ is $0, \infty$ or a root of unity for $1\leq i\leq 5$. Since
 $\varphi(\mathfrak z)$ is a bijection of $\widehat{\mathbb{C}}$, there is at most one $t^i$ such that $\varphi(t^i)=0$ and at most one $t^i$ such that $\varphi(t^i)=\infty$.
That means, there are at least three $t^i$ such that $|\varphi(t^i)|=1$.
 Since a M\"{o}bius transformation is determined by any 3 distinct points, mapping 3 distinct points from $S^1$ to $S^1$ implies that
 this $\varphi(\mathfrak z)$ maps $S^1$ homeomorphically onto $S^1$.

A M\"{o}bius transformation mapping 3 distinct points from $S^1$ to $S^1$ has a special form
$\mathcal{M}(\lambda, e^{\frak i\theta})$:
${\mathfrak z} \mapsto e^{\frak i\theta}\dfrac{\mathfrak z+\lambda}{1+\bar{\lambda}\mathfrak z}$,
where $|\lambda|\neq 1$.
%Since the inner matrix has full rank and is not diagonal or anti-diagonal matrix, by the symmetry of the three inner pairs, we can assume that $c\neq 0$.
By normalization in $f$, we may assume $z=1$.
 Comparing coefficients with $\varphi(\mathfrak z)$ we have
 $c= e^{\frak i\theta}$,
$d = e^{\frak i\theta} \lambda$ and
$w = \bar{\lambda}$.
Thus $M(f)=\left[\begin{smallmatrix}
a & 0 & 0 & b\\
0 & e^{\frak i\theta} & e^{\frak i\theta}\lambda & 0\\
0 & \bar{\lambda} & 1 & 0\\
y & 0 & 0 & a\\
\end{smallmatrix}\right]$.
Note that
$M_{x_3x_4, x_2x_1}(f)=\left[\begin{smallmatrix}
a & 0 & 0 & y\\
0 & \bar{\lambda} & e^{\frak i\theta}  & 0\\
0 & 1 & e^{\frak i\theta}\lambda  & 0\\
b & 0 & 0 & a\\
\end{smallmatrix}\right]$, obtained from $M(f)=M_{x_1x_2,x_3x_4}(f)$
by exchanging the two middle columns of $(M(f))^{T}$.
%first taking its transpose and then exchange two middle columns.
By taking two copies of $f$ and connecting
the variables $x_3, x_4$ of the first copy to the variables $x_3, x_4$ of the second copy using $(\neq_2)$,
we get a signature
 $f_1$ with the signature matrix
\[
M(f_1)=M(f)NM_{x_3x_4, x_2x_1}(f)=
\left[\begin{smallmatrix}
2ab & 0 & 0 & a^2+by\\
0 & e^{\frak i\theta}(1+|\lambda|^2) & 2e^{2\frak i\theta}\lambda & 0\\
0 &  2\bar{\lambda}  & e^{\frak i\theta}(1+|\lambda|^2) & 0\\
a^2+by & 0 & 0 & 2ay\\
\end{smallmatrix}\right].
\]
Then up to the nonzero scalar $s=e^{\frak i\theta}(1+|\lambda|^2)$,
and denote by  $\delta = 
\dfrac{2e^{\frak i\theta}\lambda}{1+|\lambda|^2}$,
we have $\bar{\delta} =
\dfrac{2e^{-\frak i\theta}\bar{\lambda}}{1+|\lambda|^2}$, 
and 
  the signature $f_1$ has the signature matrix
$M(f_1)=\left[\begin{smallmatrix}
\frac{2ab}{s} & 0 & 0 & \frac{a^2+by}{s}\\
0 & 1 & \delta & 0\\
0 & \bar{\delta} & 1 & 0\\
\frac{a^2+by}{s} & 0 & 0 & \frac{2ay}{s}\\
\end{smallmatrix}\right]$.
The inner matrix
$\left[\begin{smallmatrix}
1 & \delta\\
\bar{\delta} & 1
\end{smallmatrix}\right]$ of $M(f_1)$ is 
the product of three nonsingular $2 \times 2$ matrices, thus 
it is also nonsingular.
The two eigenvalues of
$\left[\begin{smallmatrix}
1 &  \delta \\
\bar{\delta} & 1
\end{smallmatrix}\right]$
 are $1 + |\delta|$ and $1- |\delta|$, both are real and must be nonzero.
In particular $|\delta| \not =1$.
Obviously $|{1+ |\delta|}| \neq  |{1- |\delta|}|$.
This implies that
 there are no integer $n> 0$ and complex number $\mu$ such that
$\left[\begin{smallmatrix}
1 &  {\delta} \\
  \bar{\delta} & 1
\end{smallmatrix}\right]^n=\mu I$,
i.e., $\left[\begin{smallmatrix}
1 &  \delta \\
\bar{\delta} & 1
\end{smallmatrix}\right]$ has infinite projective order.
Note that
$\left[\begin{smallmatrix}
1 &  \delta \\
\bar{\delta} & 1
\end{smallmatrix}\right]$
defines a M\"{o}bius transformation $\psi({\mathfrak z})$
of the form
$\mathcal{M}(\lambda, e^{{\frak i}\theta})$ with $\lambda = \delta$
and $\theta =0$:
${\mathfrak z} \mapsto \psi({\mathfrak z})=
\dfrac{{\mathfrak z}+\delta}{1+\bar{\delta}{\mathfrak z}}$,
mapping  $S^1$ to $S^1$.
%
%Denote $\left[\begin{smallmatrix}
%\bar{\delta} & 1\\
%1 & \delta\\
%\end{smallmatrix}\right]^n$
%by $\left[\begin{smallmatrix}
%d_n & c_n\\
%z_n & w_n\\
%\end{smallmatrix}\right]$.
%Since $\left[\begin{smallmatrix}
%d_n & c_n\\
%z_n & w_n\\
%\end{smallmatrix}\right]$ has full rank,
%$\psi^{(n)}(\mathfrak z)=\frac{w_n\mathfrak z + z_n}{c_n\mathfrak z + d_n}$
%is a M\"{o}bius transformation mapping $S^1$ to $S^1$.

We can connect the binary signature
$g_i(x_1, x_2)$ via $N$ to $f_1$. This gives us
the binary signatures  (for $1 \leq i \leq 5$)
$$h^{(1)}_i=M(f_1)Ng_i=
\left[\begin{smallmatrix}
* & 0& 0& *\\
0 & 1 &  \delta & 0\\
0 & \bar{\delta}& 1 & 0\\
* & 0& 0& *\\
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
0\\
t^i\\
1\\
0\\
\end{smallmatrix}\right]
=C_{(i, 0)}\left[\begin{smallmatrix}
0\\
\psi(t^i)\\
1\\
0\\
\end{smallmatrix}\right],
$$
where
$\psi({\mathfrak z})$ is the 
 M\"{o}bius transformation
defined by
 the matrix
$\left[\begin{smallmatrix}
1 &  {\delta} \\
\bar{\delta}  & 1
\end{smallmatrix}\right]$,
and $C_{(i, 0)} = 1 + \bar{\delta} t^i$.
Since $\psi$ maps $S^1$ to $S^1$, and $|t^i| =1$,
clearly $C_{(i, 0)} \not =0$, and
$\psi(t^i) \in S^1$.

Now we can use $h^{(1)}_i(x_2, x_1)
= (0, 1, \psi(t^i), 0)^{T}$ in place of
$g_i(x_1, x_2) = (0, 1, t^i, 0)^{T}$
and repeat this construction. Then we get
\[
h^{(2)}_i=
\left[\begin{smallmatrix}
* & 0& 0& *\\
0 & 1 &  \delta & 0\\
0 & \bar{\delta}& 1 & 0\\
* & 0& 0& *\\
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
0\\
\psi(t^i)\\
1\\
0\\
\end{smallmatrix}\right]
=C_{(i, 1)}\left[\begin{smallmatrix}
0\\
\psi^2(t^i)\\
1\\
0\\
\end{smallmatrix}\right],
\]
where $\psi^2$ is the composition $\psi \circ \psi$,
corresponding to
$\left[\begin{smallmatrix}
1 &  {\delta} \\
\bar{\delta}  & 1
\end{smallmatrix}\right]^2$,
and $C_{(i, 1)} = 1 + \bar{\delta} \psi(t^i) \not =0$.

We can iterate this process and get polynomially many
 $h^{(k)}_i = (0, \psi^k(t^i), 1, 0)^{T}$
for $1 \le i \le 5$ and $k \ge 1$.



If for each $i\in\{1, 2, 3\}$, there is some $n_i > 0$ such that
$\psi^{n_i}(t^i)=t^i$,  then $\psi^{n_0}(t^i)=t^i$,
 for $n_0=n_1n_2n_3 >0$,
and all $1\leq i\leq 3$, i.e., the M\"{o}bius transformation $\psi^{n_0}$
 fixes three distinct
complex numbers $t, t^2, t^3$. 
So the M\"{o}bius transformation is the identity map, i.e.,
$\psi^{n_0}(\mathfrak z)=\mathfrak z$ for all $\mathfrak z\in\mathbb{C}$.
This implies that $\left[\begin{smallmatrix}
1 & \delta\\
\bar{\delta} & 1
\end{smallmatrix}\right]^{n_0}=C\left[\begin{smallmatrix}
1 & 0\\
0 & 1 &
\end{smallmatrix}\right]$ for some constant $C$. 
This contradicts the fact that
$\left[\begin{smallmatrix}
1 & \delta\\
\bar{\delta} & 1
\end{smallmatrix}\right]$ does not have finite projective order.
Therefore, there is an $i \in \{1,2,3\}$
such that $\psi^{n}(t^i) \not = t^i$ for all  $n\in\mathbb{N}$.
This implies that
 $(1, \psi^{n}(t^i))$ are all distinct for $n\in\mathbb{N}$,
since $\psi$ maps $S^1$  1-1 onto $S^1$.
Then we can generate polynomially many distinct binary signatures
of the form $(0, 1, \psi^{n}(t^i), 0)^T$. By interpolation, for any $u\in\mathbb{C}$ we have
$\operatorname{Holant}(\neq_2 | f, (0, 1, u, 0)^T)\leq^p_{\operatorname{T}}\operatorname{Holant}(\neq_2 | f, g).$
\end{proof}




==> 6main-s.tex <==
\section{Using M\"{o}bius Transformations to Achieve Dichotomy}
\begin{lemma}\label{with-any-binary}
Let $f$ be a signature with matrix
$M(f)=\left[\begin{smallmatrix}
a & 0 & 0 & b\\
0 & c & d & 0\\
0 & w & z & 0\\
y & 0 & 0 & a\\
\end{smallmatrix}\right]$, where $abyczdw\neq 0$, and
$\left[\begin{smallmatrix}
 c & d \\
 w & z \\
\end{smallmatrix}\right]$ has full rank.
If  $t^i$ are distinct for $1\leq i\leq 5$,
then
$\operatorname{Holant}(\neq_2|f, (0, 1, t, 0)^T)$ is \#$\operatorname{P}$-hard.
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Proof Sketch: }
By Lemma~\ref{non:root:of:unity} and Lemma~\ref{construct-binary}, for any $u\in\mathbb{C}$, the binary signature $(0, 1, u, 0)^T$ is available.

By a normalization in $f$, we may assume that $c=1$, and by doing binary modifications to the variables $x_1, x_3$ of $f$ by $(0, 1, w^{-1}, 0)^T$
and $(0, 1, d^{-1}, 0)^T$ respectively (see subsection~\ref{subsec:Gadget-Construction}), we get a
 signature $f_1$ with signature matrix
$M(f_1)=\left[\begin{smallmatrix}
a & 0 & 0 & \frac{b}{d}\\
0 & 1 & 1 & 0\\
0 & 1 & \frac{z}{dw} & 0\\
\frac{y}{w} & 0 & 0 & \frac{a}{dw}\\
\end{smallmatrix}\right]$.
Note that $\frac{z}{dw}\neq 1$ since the inner matrix of $M(f)$ has full rank.
 \newline
 \textbf{Case A:}
For $\frac{z}{dw}\neq -1$ or $\frac{by}{dw}\neq \pm 1$,
%$\frac{z}{dw}\neq -1$ or $\left(\frac{b}{d}\right) \left(\frac{y}{w}
%\right)\neq \pm 1$,
 we can do binary modifications to $f_1$ by carefully choosing binary signatures
$(0, 1, u, 0)^T$ to get a 4-ary signature $f_2$.
Then by connecting $f_1$ and $f_2$, we can get a 4-ary signature $f_3$ that is in
Case \uppercase\expandafter{\romannumeral1},  so Holant$(\neq_2|f_3)$ is $\#$P-hard.
Thus Holant$(\neq_2|f)$ is $\#$P-hard. We omit the details here.

Now we can assume that $\frac{z}{dw}= -1$ and $\frac{by}{dw}=\pm 1$.
 We prove the lemma for
 $\frac{z}{dw}=-1$, $\frac{by}{dw}=-1$.
 The proof for $\frac{z}{dw}=-1$, $\frac{by}{dw}=1$ is similar.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newline
 \textbf{Case B:}
 Suppose $\frac{z}{dw}=-1$, $\frac{by}{dw}=-1$, and $\frac{a^2}{dw}\neq 1$.
By the symmetry of the three pairs we have
 %By symmetry of the three inner pairs,
 $M_{x_1x_4, x_2x_3}(f_1)=\left[\begin{smallmatrix}
 a & 0 & 0 & 1\\
 0 & 1 & \frac{b}{d} & 0\\
 0 & \frac{y}{w} & -1 & 0\\
 1 & 0 & 0 & \frac{a}{dw}\\
\end{smallmatrix}\right]$.
By doing modifications to $M_{x_1x_4, x_2x_3}(f_1)$ using binary signatures
$(0, 1, \frac{w}{y}, 0)^T$ and $(0, 1, \frac{d}{b}, 0)^T$, we get the signature
 $f_4$
 whose signature matrix is
 $M(f_4)=\left[\begin{smallmatrix}
 a & 0 & 0 & \frac{d}{b}\\
 0 & 1 & 1 & 0\\
 0 & 1 & 1 & 0\\
 \frac{w}{y} & 0 & 0 & \frac{a}{by}\\
\end{smallmatrix}\right]$.
Note that the entry
$f_4(1,1,1,1) = \frac{a}{dw} \cdot  \frac{w}{y} \cdot \frac{d}{b} =
\frac{a}{by}$.
 Note that $f_4$
 is a redundant signature and
its compressed signature matrix
$\left[\begin{smallmatrix}
 a & 0 & \frac{d}{b}\\
 0 & 1 & 0\\
\frac{w}{y} & 0 & \frac{a}{by}\\
\end{smallmatrix}\right]$
has full rank by $a^2 \not = dw$. Thus
% and $by=-dw$. Thus
Holant$(\neq_2|f_4)$ is \#P-hard by Theorem~\ref{redundant}.
It follows that Holant$(\neq_2|f, (0, 1, t, 0)^T)$ is \#P-hard.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newline
 \textbf{Case C:}
Suppose $\frac{z}{dw}=-1$, $\frac{by}{dw}=-1$, $\frac{a^2}{dw}=1$.
%By Lemma~\ref{normalize:a=x}, we can assume that $M_{x_1x_4, x_2x_3}(f_1)=\left[\begin{smallmatrix}
%1 & 0 & 0 & 1\\
%0 & 1 & \frac{b}{d} & 0\\
%0 & \frac{y}{w} & -1 & 0\\
%1 & 0 & 0 & 1\\
%\end{smallmatrix}\right]$.
In this case
$M_{x_1x_2,x_3x_4}(f_1)
=\left[\begin{smallmatrix}
a & 0 & 0 & \frac{b}{d}\\
0 & 1 & 1 & 0\\
0 & 1 & -1 & 0\\
-\frac{d}{b} & 0 & 0 & \frac{1}{a}
\end{smallmatrix}\right]$.
By the symmetry of three pairs we have
$M_{x_1x_4,x_3x_2}(f_1) = \left[\begin{smallmatrix}
a & 0 & 0 & 1\\
0 & 1 & \frac{b}{d} & 0\\
0 & -\frac{d}{b} & -1 & 0\\
1 &  0 & 0 & \frac{1}{a}
\end{smallmatrix}\right]$.
By doing binary modifications to the variables $x_1, x_3$ of this function
 using $(0, 1, -\frac{b}{d}, 0)^T$ and $(0, 1, \frac{d}{b}, 0)^T$
respectively, we get a signature $f_5$ with signature matrix
$M(f_5)=\left[\begin{smallmatrix}
a & 0 & 0 & \frac{d}{b}\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
-\frac{b}{d} & 0 & 0 & -\frac{1}{a}\\
\end{smallmatrix}\right]$.
By connecting two copies of $f_5$ via $N$, we get a signature $f_6$ whose signature matrix is
\[M(f_6)=M(f_5)NM_{x_3x_4, x_1x_2}(f_5)=\left[\begin{smallmatrix}
a & 0 & 0 & \frac{d}{b}\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
-\frac{b}{d} & 0 & 0 & -\frac{1}{a}\\
\end{smallmatrix}\right]N\left[\begin{smallmatrix}
a & 0 & 0 & -\frac{b}{d}\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
\frac{d}{b} & 0 & 0 & -\frac{1}{a}\\
\end{smallmatrix}\right]=2\left[\begin{smallmatrix}
\frac{ad}{b} & 0 & 0 & -1\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
-1 & 0 & 0 & \frac{b}{ad}
\end{smallmatrix}\right].\]
%By Lemma~\ref{normalize:a=x}, we can assume that $f_7$ has the signature matrix $M(f_7)=\left[\begin{smallmatrix}
%1 & 0 & 0 & -1\\
% & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%-1 & 0 & 0 & 1
%\end{smallmatrix}\right]$.
Then by connecting two copies of $f_6$ via $N$, we get a signature $f_7$ whose signature matrix is
\[
M(f_7)=
M(f_6)NM(f_6)=4\left[\begin{smallmatrix}
\frac{ad}{b} & 0 & 0 & -1\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
-1 & 0 & 0 & \frac{b}{ad}
\end{smallmatrix}\right]N\left[\begin{smallmatrix}
\frac{ad}{b} & 0 & 0 & -1\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
-1 & 0 & 0 & \frac{b}{ad}
\end{smallmatrix}\right]=8\left[\begin{smallmatrix}
-\frac{ad}{b} & 0 & 0 & 1\\
0 & 1 & 1 & 0\\
0 & 1 & 1 & 0\\
1 & 0 & 0 & -\frac{b}{ad}
\end{smallmatrix}\right].
\]
Now the important point is that $f_7$ is a \emph{symmetric}
signature where all  weight 2 entries are equal.
Thus,  after the nonzero scalar 8,
$f_7=[s, 0, 1, 0, \frac{1}{s}]$ written as a symmetric
signature listing the values of $f_7$ according to its Hamming weight,
and where $s=-\frac{ad}{b}\neq 0$.

Now we have the reduction Holant$(\neq_2|f_7, (0, 1, u, 0)^T)\leq_T^p$Holant$(\neq_2|f, (0, 1, t, 0)^T)$ for any $u\in\mathbb{C}$.
We finish the proof for this case by proving that  Holant$(\neq_2|f_7, (0, 1, u, 0)^T)$ is \#P-hard for a carefully
chosen $u$.
Let $T=\left[\begin{smallmatrix}
1 & \sqrt{s}\\
 \frak i  & -\frak i\sqrt{s}
\end{smallmatrix}\right]
= \left[\begin{smallmatrix}
1 & 1\\
 \frak i  & -\frak i
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
1 & 0 \\
0 & \sqrt{s}
\end{smallmatrix}\right]
=\left[\begin{smallmatrix}
1 & 0 \\
0 & \frak i
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
1 & 1\\
1 & -1
\end{smallmatrix}\right]
\left[\begin{smallmatrix}
1 & 0 \\
0 & \sqrt{s}
\end{smallmatrix}\right]$.
%=\sqrt{2}Z
%\left[\begin{smallmatrix}
%1 & 0 \\
%0 & \sqrt{s}
%\end{smallmatrix}\right]$.
By the holographic transformation using $T$,
note that $(\ne_2) (T^{-1})^{\otimes 2}$
and $T^{\otimes 4} f_7$ are
nonzero scalar multiples of $(=_2)$ and $(=_4)$ respectively,
 we have
$
\operatorname{Holant}(\neq_2|f_7, (0, 1, u, 0)^T)\equiv^p_{T}\operatorname{Holant}(=_2|=_4, T^{\otimes 2}(0, 1, u, 0)^T)
$.
We can calculate that
 $g=T^{\otimes 2}(0, 1, u, 0)^T=\sqrt{s}(u+1, (u-1)\frak i, (1-u)\frak i, u+1)^T$.
By $=_2$ on the left side and $=_4$ on the right side, we can construct $=_{2k}$ for any $k\in\mathbb{N}$.
This implies that
\[
\operatorname{\#CSP}^2(g)\leq_T^p\operatorname{Holant}(=_2|=_4, g).
\]
Let $u=3$, then  $g\notin\mathscr{P}\cup\mathscr{A}\cup\alpha\mathscr{A}\cup\mathscr{L}$. Thus \#CSP$^2(g)$ is \#P-hard
by Theorem~\ref{CSP2}.
Hence Holant$(\neq_2|f_7, (0, 1, u, 0)^T)$ is \#P-hard and Holant$(\neq_2|f, (0, 1, t, 0)^T)$ is \#P-hard.




\begin{theorem}\label{with:(0,1,0,0)}
If $f$ has the signature matrix
$M(f)=\left[\begin{smallmatrix}
a & 0 & 0 & b\\
0 & c & d & 0\\
0 & w & z & 0\\
y & 0 & 0 & a\\
\end{smallmatrix}\right]$ where $abyczdw\neq 0$ and
$\left[\begin{smallmatrix}
 c & d \\
 w & z \\
\end{smallmatrix}\right]$ has full rank, then
$\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard, or $f$ is  $\mathscr{A}$-transformable.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
By a normalization in $f$, we may assume that $c=1$.
For any $u\in\{b, y, d, w\}$, we can get $(0, 1, u, 0)^T$ by doing a
loop to some two variables of $f$ using $(0, 1, 0, 0)^T$ via $N$.
Thus if  there exists $u\in\{b, y, d, w\}$ such that $u^i$ are distinct for $1\leq i\leq 5$, then
$\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
So we may assume  all of $\{b, y, d, w\}$ are in $\{\pm 1, \pm \frak i, \omega, \omega^2\}$,
where $\omega = e^{2 \pi {\frak i}/3}$.
%where $\omega^3=1$ and $\omega\neq 1$.
%Then by doing loops to $f$ using $g=(0, 1, 0, 0)^{T}$,
%we can get binary signatures
% $h_1=M_{x_3x_4, x_1x_2}(f)g=(0, 1, d, 0)^T,$
%$ h_2=M(f)g=(0, 1, w, 0),$
% $ h_3=M_{x_1x_2, x_4x_3}(f)g=d(0, 1,\frac{z}{d}, 0), $
%$h_4=M_{x_2x_3, x_1x_4}(f)g=(0, 1, b, 0),$
%h_5=M_{x_1x_4, x_2x_3}(f)g=(0, 1, y, 0)$.

Note that  for any $u\neq 0$, if we have $g(x_1, x_2)=(0, 1, u, 0)^T$, then
we also
have $g'(x_1, x_2)=g(x_2, x_1)=u(0, 1, u^{-1}, 0)^T$, i.e., we have $(0, 1, u^{-1}, 0)^T$ after the nonzero scalar $u$.
%
%can construct $(0, 1, u^{-1}, 0)^T$.
%If $u$ is not a root of unity, then we can get $(0, 1, u^{-1}, 0)^T$ by interpolation.
%If $u$ is a root of unity of order $d$, by linking $d-1$ copies of $(0, 1, u, 0)^T$,
%we get $(0, 1, u^{d-1}, 0)^T=(0, 1, u^{-1}, 0)^T$.%
%
%Since we have $(0, 1, d, 0)^T$, $(0, 1, w, 0)^T$  by doing loops to $f$ using $(0, 1, 0, 0)^T$,
So we have $(0, 1, d^{-1}, 0)^T$
and $(0, 1, w^{-1}, 0)^T$.
By binary modifications using  $(0, 1, w^{-1}, 0)^T$
and $(0, 1, d^{-1}, 0)^T$ to the variables
$x_1, x_3$ of $f$ respectively, we get a signature $f_1$ whose signature matrix is
$M(f_1)=\left[\begin{smallmatrix}
a & 0 & 0 & \frac{b}{d}\\
0 & 1 & 1 & 0\\
0 & 1 & \frac{z}{dw} & 0\\
\frac{y}{w} & 0 & 0 & \frac{a}{dw}\\
\end{smallmatrix}\right]$.
Since  $\left[\begin{smallmatrix}
 1 & d\\
 w & z \\
\end{smallmatrix}\right]$ has full rank, we have $\frac{z}{dw}\neq 1$.
By doing a loop to $f_1$ using $\neq_2$, we get the
 binary signature  $h=M(f)(\neq_2)=(0, 2, 1+\frac{z}{dw}, 0)^T$.

We claim that $\frac{z}{dw}=-1$ or we are done.
By doing a loop to $f_1$ using $(0, 1, 0, 0)^T$, we have $(0, 1, \frac{z}{dw}, 0)^T$.
If $(\frac{z}{dw})^i$ are distinct for $1\leq i\leq 5$, then
the problem
$\operatorname{Holant}(\neq_2|f, (0, 1, \frac{z}{dw}, 0)^T)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
 Thus $\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard.
 So we may assume
 that $\frac{z}{dw}\in\{-1, \frak i, -\frak i, \omega, \omega^2\}$.
 If $\frac{z}{dw}=\frak i$ or $-\frak i$, then $|1+\frac{z}{dw}|=\sqrt{2}$.
 If $\frac{z}{dw}=\omega$ or $\omega^2$, then $|1+\frac{z}{dw}|=1 \not = 2$.
 So
 $\operatorname{Holant}(\neq_2|f, h)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
 Thus $\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0))^T$ is $\#\operatorname{P}$-hard.
 So we may assume that $(0, 1, \frac{z}{dw}, 0)^T=(0, 1, -1, 0)^T$.


%If there exists $u\in\{b, y, \frac{z}{d}, d, w\}$ such that $u^i$ are distinct for $1\leq i\leq 5$, then
%$\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
%Thus all of them are roots of unity and the orders are less than 5.

Suppose there exists  $u\in\{b, d, y,  w\}$
such that $u=\omega$ or $\omega^2$.
By linking $(0, 1, u, 0)^T$ and $(0, 1, -1, 0)^T$ using $\neq_2$, we get
the binary signature $(0, 1, -u, 0)^T$.
Note that $(-u)^i$ are distinct for $1\leq i\leq 6$, therefore
$\operatorname{Holant}(\neq_2|f, (0, 1, -u, 0)^T)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
It follows that  $\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard.
%If there exists  $v\in\{b, y, d, w\}$
%such that $v\neq 1, v^3\neq 1$, i.e., $v\in\{-1, \frak{i}, -\frak{i}\}$.
%hen by connecting $(0, 1, u, 0)^T$ and $(0, 1, v, 0)^T$ using $\neq_2$, we get $(0, 1, uv, 0)^T$.
%Note that the order of $uv$ is greater than 4.
%$\operatorname{Holant}(\neq_2|f, (0, 1, uv, 0)^T)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
%hus $\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard.
%therwise,  all of $\{b, y, d, w\}$ are 3-th roots of unity.
%\begin{itemize}
%\item If $z^3=1$, then $(\frac{z}{dw})^3=1$.
%ince $\frac{z}{dw}\neq 1$, $\frac{z}{dw}=\omega$ or $\omega^2$.
%In each case, we have
%$|1+\frac{z}{dw}|=1$. Note that $h=M(f_1)(\neq_2)=2(0, 1, t,  0)^T$, where
%$t=\frac{1+\frac{z}{dw}}{2}\neq 0$ is not a root of unity.
%Thus $\operatorname{Holant}(\neq_2|f, h)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
%If follows that $\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard.
%item If $z^3\neq 1$, then $(\frac{z}{dw})^3\neq 1$.
%By doing a loop to $f_1$ using $(0, 1, 0, 0)^T$, we have $(0, 1, \frac{z}{dw}, 0)^T$.
%f $(\frac{z}{dw})^i$ are distinct for $1\leq i\leq 5$, then  $\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard
%by  Lemma~\ref{with-any-binary}.
%Otherwise, $\frac{z}{dw}\in\{-1, \frak i, -\frak i\}$.
%Then by linking $(0, 1, \frac{z}{dw}, 0)^T$ and $(0, 1, u, 0)^T$, we get the binary signature
%(0, 1, \frac{z}{dw}u, 0)^T$.
%Note that $\frac{z}{dw}u$ is a root of unity of order greater than 4. Thus
%$\operatorname{Holant}(\neq_2|f, (0, 1, \frac{z}{dw}u, 0)^T)$ Lemma~\ref{with-any-binary}.
%Then
%$\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#\operatorname{P}$-hard.
%\end{itemize}
%
%Thus $f$ has the signature matrix
%$\left[\begin{smallmatrix}
% & 0 & 0 & \omega_1\\
%0 & 1 & \omega_2 & 0\\
%0 & \omega_3 & z & 0\\
%\omega_4 & 0 & 0 & a\\
%\end{smallmatrix}\right]$, where $w_i^3=1$ for $1\leq i\leq 4$.
%ote that $h=(0, 2, 1+\frac{z}{\omega_2\omega_3}, 0)^T$ in this case and $\frac{z}{\omega_2\omega_3}\neq 1$.
%If $\frac{z}{\omega_2\omega_3}= -1$, then we have $(0, 1, -1, 0)^T$ by doing a loop to $f_1$ using $(0, 1, 0, 0)^T$.
%By connecting $(0, 1, -1, 0)^T$ to $(0, 1, u, 0)^T$, we get the binary signature $(0, 1, -u_0, 0)^T$.
%Since the order of $-u_0$ is 6, we prove hardness by Lemma~\ref{with-any-binary}.
%Otherwise, $\frac{z}{\omega_2\omega_3}\neq \pm 1$,
%So since $|1+\frac{z}{\omega_2\omega_3}|\neq 0, 2$,
%$\operatorname{Holant}(\neq_2|f, h)$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.
%hus
% $\operatorname{Holant}(\neq_2|f, (0, 1, 0, 0))^T$ is $\#\operatorname{P}$-hard by Lemma~\ref{with-any-binary}.%


Now we can assume
$\{b, y, d,  w\}\subseteq\{1, -1, \frak{i}, -\frak{i}\}$.
Then by $\frac{z}{dw}=-1$, we have $z^4=1$.
Thus $\{b, y, z, d,  w\}\subseteq\{1, -1, \frak{i}, -\frak{i}\}$.
  There exist
  $j, k,  \ell, m, n\in\{0, 1, 2, 3\}$, such that
\[b=\frak{i}^{j},~~~ y=\frak{i}^{k},~~~ z=\frak{i}^{\ell}, ~~~
  d=\frak{i}^{m}, ~~~ w=\frak{i}^{n}.\]
%So $h_i$ are affine signatures for $1\leq i\leq 5$.
The signature matrices of $f$ and $f_1$ are respectively
$$M(f)=\left[\begin{smallmatrix}
a & 0 & 0 & \frak{i}^{j}\\
0 & 1 & \frak{i}^{m} & 0\\
0 & \frak{i}^{n} & \frak{i}^{\ell} & 0\\
\frak{i}^{k}& 0 & 0 & a
\end{smallmatrix}\right],~~~~\mbox{and}~~~~
M(f_1)=\left[\begin{smallmatrix}
a & 0 & 0 & \frak{i}^{j-m}\\
0 & 1 & 1 & 0\\
0 & 1 & \frak{i}^{\ell-m-n} & 0\\
\frak{i}^{k-n}& 0 & 0 & a\frak i^{-m-n}
\end{smallmatrix}\right].$$
We have $\ell-m-n\equiv 2 \pmod 4$ by $\frac{z}{dw}=\frak{i}^{\ell-m-n}=-1$.

Note that $M_{x_1x_4, x_3x_2}(f)=
\left[\begin{smallmatrix}
a & 0 & 0 & \frak{i}^{m}\\
0 & 1 & \frak{i}^{j} & 0\\
0 & \frak{i}^{k} & \frak{i}^{\ell} & 0\\
\frak{i}^{n}& 0 & 0 & a
\end{smallmatrix}\right]$.
By doing a loop to $f$ using $(0, 1, \frak i^{-k}, 0)^T$, we get the binary signature
$(0, 2, \frak i^{j}(1+\frak i^{\ell-j-k}), 0)^T$.
If $\ell-j-k\equiv 1 \pmod 2$, then $|\frak{i}^{j}(1+\frak{i}^{\ell-j-k})|
= \sqrt{2}$ and
%\neq 2, 0$ and
Holant$(\neq_2|f, (0, 2, \frak{i}^{j}(1+\frak{i}^{\ell-j-k}), 0)^T)$ is $\#$P-hard
by Lemma~\ref{with-any-binary}.
Thus Holant$(\neq_2|f, (0, 1, 0, 0)^T)$ is $\#$P-hard.
Hence  we have $\ell-j-k\equiv 0 \pmod 2$.
By $\ell-m-n\equiv 2 \pmod 4$, we have
\[ j+k + m+n \equiv 0 \pmod 2.\]




By connecting two copies of $f$, we get a signature $f_2$ whose signature matrix is
\[M(f_2)=M(f)NM_{x_3x_4, x_1x_2}(f)=
\left[\begin{smallmatrix}
2a\frak{i}^{j} & 0 & 0 & a^2+\frak{i}^{j+k}\\
0 & 2\frak{i}^{m} & \frak{i}^{\ell}+\frak{i}^{m+n} & 0\\
0 & \frak{i}^{\ell}+\frak{i}^{m+n} & 2\frak{i}^{n+\ell} & 0\\
a^2+\frak{i}^{j+k} & 0 & 0 & 2a\frak{i}^{k}
\end{smallmatrix}\right].
\]
Note that $\frak{i}^{\ell}+\frak{i}^{m+n}=0$ by $\ell-m-n\equiv 2 \pmod 4$.
If $a^2+\frak{i}^{j+k}\neq 0$, then $f_2$ is in Case \uppercase\expandafter{\romannumeral1}
and
Holant$(\neq_2|f_2)$ is $\#$P-hard.
Thus Holant$(\neq_2|f)$ is $\#$P-hard.

Otherwise, $a^2+\frak{i}^{j+k}=0$. Then $M(f)=\left[\begin{smallmatrix}
\frak{i}^{\frac{j+k}{2}+\epsilon} & 0 & 0 & \frak{i}^{j}\\
0 & 1 & \frak{i}^{m} & 0\\
0 & \frak{i}^{n} & \frak{i}^{\ell} & 0\\
\frak{i}^{k}& 0 & 0 & \frak{i}^{\frac{j+k}{2}+\epsilon}
\end{smallmatrix}\right]$, where $\epsilon=\pm 1$.
Let $r =j+m$.
We apply a holographic transformation
defined by
$\left[\begin{smallmatrix}
 1 & 0\\
 0 & \gamma
\end{smallmatrix}\right]$, where $\gamma^2=\frak{i}^{\frac{j+k}{2}+r+\epsilon}$, then we get
$
\operatorname{Holant}(\neq_2|f)\equiv^p_{T}\operatorname{Holant}(\neq_2|\widehat{f}),
$
where $\widehat{f}=\left[\begin{smallmatrix}
 1 & 0\\
 0 & \gamma
\end{smallmatrix}\right]^{\otimes 4}f$, whose signature matrix is
$M(\widehat{f})=\frak{i}^{\frac{j+k}{2}+\epsilon}\left[\begin{smallmatrix}
1 & 0 & 0 & \frak{i}^{j+r}\\
0 & \frak i^{r} & \frak{i}^{m+r} & 0\\
0 & \frak{i}^{n+r} & \frak{i}^{\ell+r} & 0\\
\frak{i}^{k+r}& 0 & 0 & -\frak{i}^{j+k+2r}
\end{smallmatrix}\right]$.
%%% that - in -\frak{i}^{j+k+2r} comes from i^{2 epsilin}
By $\ell \equiv m+n+ 2 \pmod 4$, we have
% $\ell+r+1\equiv r+m+n+3 \pmod 4$.
%Let $k\equiv n+s\pmod 4$, where $s\in\{0, 1, 2, 3\}$.
%Then
\[M(\widehat{f})=\frak{i}^{\frac{j+k}{2}+\epsilon}\left[\begin{smallmatrix}
1 & 0 & 0 & \frak{i}^{j+r}\\
0 & \frak i^{r} & \frak{i}^{m+r} & 0\\
0 & \frak{i}^{n+r} & -\frak{i}^{m+n+r} & 0\\
\frak{i}^{k+r}& 0 & 0 & -\frak{i}^{j+k+2r}
\end{smallmatrix}\right].\]
This function is an affine function; indeed
 let
\[Q(x_1, x_2, x_3)=(k-n-r)x_1x_2+(2j+2)x_1x_3+(2j)x_2x_3+(n+r)x_1+rx_2+(j+r)x_3,\]
then
 $\widehat{f}(x_1, x_2, x_3, x_4)=\frak{i}^{\frac{j+k}{2}+\epsilon}\cdot
\frak{i}^{Q(x_1, x_2, x_3)}$ on the support
of $\widehat{f}$: $x_1 + x_2 + x_3 + x_4 \equiv 0 \pmod 2$.
 Moreover, $k-n-r \equiv j + k + n + m \equiv 0 \pmod 2$,
all cross terms have even coefficients.
% we have $s-r\equiv k+n+j+m\pmod 2$ by $j+k\equiv m+n\pmod 2$ and
% $m-j-r+2\equiv -2j+2\pmod 2$.
% This implies
% that the coefficients of the cross terms of $Q$ are even.
Thus $\widehat{f}\in\mathscr{A}$.
\end{proof}

%****************************
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 %$r_3+r_5+1\equiv 0\pmod 2$ iff $r_1+r_2+1\equiv 0 \pmod 2$.
%We prove that $\widehat{f}$ is in $\mathscr{A}$.
%\newline
% \textbf{Case A:} For $r_3+r_5+1\equiv 0 \pmod 4$,
%$M(\widehat{f})=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\left[\begin{smallmatrix}
%1 & 0 & 0 & \frak{i}^{r_1+1}\\
%0 & i & \frak{i}^{r_2+1} & 0\\
%0 & \frak{i}^{r_3+1} & \frak{i}^{r_4+1} & 0\\
%\frak{i}^{-r_3}& 0 & 0 & \frak{i}^{r_1-r_3-1}
%\end{smallmatrix}\right]$. Letting
%\[Q_1(x_1, x_2, x_3)=-2(1+r_3)x_1x_2+(r_2-r_1+1)x_1x_3+(r_2-r_1-1)x_2x_3+(r_3+1)x_1+x_2+(r_1+1)x_3,\]
% $\widehat{f}(x_1, x_2, x_3, x_4)=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\frak{i}^{Q_1(x_1, x_2, x_3)}$ if $(x_1, x_2, x_3, x_4)\neq 0$.
%Note that the coefficients of the cross terms of $Q_1$ are even by $r_2-r_1+1\equiv r_2+r_1+1\equiv 0\pmod 2$.
%Thus $\widehat{f}\in\mathscr{A}$.
%\newline
% \textbf{Case B:}
% For $r_3+r_5+1\equiv 2 \pmod 4$,
%$M(\widehat{f})=\frak{i}^{\frac{r_1+r_5}{2}-1}\left[\begin{smallmatrix}
%1 & 0 & 0 & \frak{i}^{r_1+1}\\
%0 & i & \frak{i}^{r_2+1} & 0\\
%0 & \frak{i}^{r_3+1} & \frak{i}^{r_4+1} & 0\\
%-\frak{i}^{-r_3}& 0 & 0 & -\frak{i}^{r_1-r_3-1}
%\end{smallmatrix}\right]$.
%Letting%
%\[Q_2(x_1, x_2, x_3)=-2r_3x_1x_2+(r_2-r_1+1)x_1x_3+(r_2-r_1-1)x_2x_3+(r_3+1)x_1+x_2+(r_1+1)x_3,\]
% $\widehat{f}(x_1, x_2, x_3, x_4)=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\frak{i}^{Q_2(x_1, x_2, x_3)}$ if $(x_1, x_2, x_3, x_4)\neq 0$.
%Note that the coefficients of the cross terms of $Q_1$ are even.
%Thus $\widehat{f}\in\mathscr{A}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%If $r_1+r_2\equiv 0 \pmod 2$, then $r_3+r_5\equiv 0 \pmod 2$.
%Then after the holographic transformation using $\left[\begin{smallmatrix}
% 1 & 0\\
% 0 & \beta
%\end{smallmatrix}\right]$ on $\widehat{f}$, where $\beta^2=-i$, we get the signature $\widehat{f'}$ whose signature matrix is
%whose signature matrix is
%$M(\widehat{f'})=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\left[\begin{smallmatrix}
%1 & 0 & 0 & \frak{i}^{r_1}\\
%0 & 1 & \frak{i}^{r_2} & 0\\
%0 & \frak{i}^{r_3} & \frak{i}^{r_4} & 0\\
%\frak{i}^{r_5}& 0 & 0 & -\frak{i}^{r_1+r_5}
%\end{smallmatrix}\right]$.
%We claim that $\widehat{f'}$ is affine by giving the quadratic polynomial for the free variables $x_1, x_2, x_3$.
%\newline
% \textbf{Case C:} For $r_3+r_5\equiv 0 \pmod 4$,
%$M(\widehat{f'})=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\left[\begin{smallmatrix}
%1 & 0 & 0 & \frak{i}^{r_1}\\
%0 & 1 & \frak{i}^{r_2} & 0\\
%0 & \frak{i}^{r_3} & -\frak{i}^{r_2+r_3} & 0\\
%\frak{i}^{-r_3}& 0 & 0 & -\frak{i}^{r_1-r_3}
%\end{smallmatrix}\right]$.
%Letting
%\[Q_3(x_1, x_2, x_3)=-2r_3x_1x_2+(r_2-r_1+2)x_1x_3+(r_2-r_1)x_2x_3+r_3x_1+r_1x_3,\]
% $\widehat{f'}(x_1, x_2, x_3, x_4)=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\frak{i}^{Q_3(x_1, x_2, x_3)}$ if $(x_1, x_2, x_3, x_4)\neq 0$.
% Note that the coefficients of the cross terms of $Q_3$ are even.
%Thus $\widehat{f'}\in\mathscr{A}$.
%\newline
 %\textbf{Case D:} For $r_3+r_5\equiv 2 \pmod 4$,
%$M(\widehat{f'})=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\left[\begin{smallmatrix}
%1 & 0 & 0 & \frak{i}^{r_1}\\
%0 & 1 & \frak{i}^{r_2} & 0\\
%0 & \frak{i}^{r_3} & -\frak{i}^{r_2+r_3} & 0\\
%-\frak{i}^{-r_3}& 0 & 0 & \frak{i}^{r_1-r_3}
%%\end{smallmatrix}\right]$.
%Thus let
%\[Q_4(x_1, x_2, x_3)=-2(r_3+1)x_1x_2+(r_2-r_1+2)x_1x_3+(r_2-r_1)x_2x_3+r_3x_1+r_1x_3,\]
%then $\widehat{f'}(x_1, x_2, x_3, x_4)=\frak{i}^{\frac{r_1+r_5}{2}-\epsilon}\frak{i}^{Q(x_1x_2x_3)}$ if $(x_1, x_2, x_3, x_4)\in$Supp$(\widehat{f'})$.
% Note that the coefficients of the cross terms of $Q_4$ are even.%
%Thus $\widehat{f'}\in\mathscr{A}$.
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\iffalse
%$\mathbf{Outline~ of ~the ~Proof:}$
%By Lemma~\ref{construct-binary},
 %$(0, 1, u, 0)^T$ is available for any $u\in\mathbb{C}$.
 %Thus we have $(0, 1, w^{-1}, 0)^T$, $(0, 1, d^{-1}, 0)^T$.
 %By normalization in $f$, we may assume that $c=1$, and $f$ has the signature matrix
%$M(f)=\left[\begin{smallmatrix}
%a & 0 & 0 & b\\
%0 & 1 & d & 0\\
%0 & w & z & 0\\
%y & 0 & 0 & a\\
%\end{smallmatrix}\right]$.
%Then by doing binary modification to the variables $x_1, x_3$ of $f$ by $(0, 1, w^{-1}, 0)^T$
%and $(0, 1, d^{-1}, 0)^T$ respectively, we get the signature $f_1$ whose signature matrix is
%$M(f_1)=\left[\begin{smallmatrix}
%a & 0 & 0 & \frac{b}{d}\\
%0 & 1 & 1 & 0\\
%0 & 1 & \frac{z}{dw} & 0\\
%\frac{y}{w} & 0 & 0 & \frac{a}{dw}\\
%\end{smallmatrix}\right]$.
%Note that $\frac{z}{dw}\neq 1$ since the inner matrix of $M(f)$ has full rank.
%If $\frac{z}{dw}\neq -1$, by doing binary modification to the variable $x_3$ of $f_1$ using  $(0, 1, -\frac{z}{dw}, 0)^T$, we have
%the signature $f_2$ whose signature matrix is
%$M(f_2)=\left[\begin{smallmatrix}
%a & 0 & 0 & -\frac{bz}{d^2w}\\
%0 & 1 & -\frac{z}{dw} & 0\\
%0 & 1 & -\frac{z^2}{d^2w^2} & 0\\
%\frac{y}{w} & 0 & 0 & -\frac{az}{d^2w^2}\\
%\end{smallmatrix}\right]$.
%Then by connecting $f_2$ and $f_1$ using $\neq_2$ we get the signature $f_3$ whose signature matrix is
%\[M(f_2)NM(f_1)=\left[\begin{smallmatrix}
%\frac{a}{w}(y-\frac{bz}{d^2}) & 0 & 0 & \frac{1}{dw}(a^2-\frac{b^2z}{d^2})\\
%0 & 1-\frac{z}{dw} & 0 & 0\\
%0 & 1-\frac{z^2}{d^2w^2} & \frac{z}{dw}(1-\frac{z}{dw}) & 0\\
%\frac{1}{w^2}(y^2-\frac{a^2z}{d^2}) & 0 & 0 & \frac{a}{dw^2}(y-\frac{bz}{d^2})\\
%\end{smallmatrix}\right].\]
%Since $\frac{z}{dw}\neq \pm 1$, there are exact three nonzero entries in the inner matrix of $M(f_3)$.
%%we have $(1-\frac{z}{dw})(1-\frac{z^2}{d^2w^2})(\frac{z}{dw}(1-\frac{z}{dw}))\neq 0$.
%Note that $f_3$ is in Case \uppercase\expandafter{\romannumeral1}, so  Holant$(\neq_2|f_3)$ is $\#$P-hard.
%Thus Holant$(\neq_2|f)$ is $\#$P-hard.%
%
%Otherwise, $\frac{z}{dw}=-1$ and
% $M(f_1)=\left[\begin{smallmatrix}
%a & 0 & 0 & \frac{b}{d}\\
%0 & 1 & 1 & 0\\
%0 & 1 & -1 & 0\\
%\frac{y}{w} & 0 & 0 & \frac{a}{dw}\\
%\end{smallmatrix}\right]$.
%\begin{itemize}
%\item For $\frac{by}{dw}\neq \pm1$, note that
%$M_{x_1x_4, x_2x_3}(f_1)=\left[\begin{smallmatrix}
%a & 0 & 0 & 1\\
%0 & 1 & \frac{b}{d} & 0\\
%0 & \frac{y}{w} & -1 & 0\\
%1 & 0 & 0 & \frac{a}{dw}\\
%\end{smallmatrix}\right]$. By doing binary modification to $x_2$ of $f_1$ using $(0, 1, \frac{d^2}{b^2}, 0)^T$, we get the signature $f_4$
%whose signature matrix is
%$M(f_4)=\left[\begin{smallmatrix}
%a & 0 & 0 & \frac{d^2}{b^2}\\
%0 & 1 & \frac{d}{b} & 0\\
%0 & \frac{y}{w} & -\frac{d^2}{b^2} & 0\\
%1 & 0 & 0 & \frac{ad}{b^2w}\\
%\end{smallmatrix}\right]$.
%Then by connecting $f_4$ and $f_1$ using $\neq_2$, we get the signature $f_5$ whose signature matrix is
%\[
%M(f_4)NM_{x_1x_4, x_2x_3}(f_1)=
%\left[\begin{smallmatrix}
%a(1+\frac{d^2}{b^2}) & 0 & 0 & \frac{a^2}{dw}+\frac{d^2}{b^2}\\
%0 & \frac{y}{w}+\frac{d}{b} & 0 & 0\\
%0 & \frac{y^2}{w^2}-\frac{d^2}{b^2} & -(\frac{y}{w}+\frac{d}{b}) & 0\\
%1+\frac{a^2d}{b^2w} & 0 & 0 & \frac{a}{dw}+\frac{ad}{b^2w}\\
%\end{smallmatrix}\right].
%\]
%Since $\frac{by}{dw}\neq \pm 1$, there are exact three nonzero entries in the inner matrix of $M(f_5)$.
%we have $(1-\frac{z}{dw})(1-\frac{z^2}{d^2w^2})(\frac{z}{dw}(1-\frac{z}{dw}))\neq 0$.
%Note that $f_5$ is in Case \uppercase\expandafter{\romannumeral1}, so Holant$(\neq_2|f_5)$ is $\#$P-hard.
%Thus Holant$(\neq_2|f)$ is $\#$P-hard.%
%\item For $\frac{by}{dw}=-1$, the inner matrix of $M_{x_1x_4, x_2x_3}(f_1)$ is degenerate.
%Note that there at most one of $\{\frac{y}{w}, \frac{b}{d}\}$ is $-1$.
%Thus if $\frac{a^2}{dw}\neq 1$, then Holant$(\neq_2|f_1)$ is \#P-hard by Lemmma~\ref{full:out:deg:inner}.
%So Holant$(\neq_2|f)$ is \#P-hard.%
%
%Otherwise, $\frac{a^2}{dw}=1$. By Lemma~\ref{normalize:a=x}, we can assume that $M_{x_1x_4, x_2x_3}(f_1)=\left[\begin{smallmatrix}
%1 & 0 & 0 & 1\\
%0 & 1 & \frac{b}{d} & 0\\
%0 & \frac{y}{w} & -1 & 0\\
%1 & 0 & 0 & 1\\
%\end{smallmatrix}\right]$.
%By doing binary modification to the variable $x_1, x_2$ of $f_1$ using $(0, 1, -\frac{b}{d}, 0)^T$ and $(0, 1, \frac{d}{b}, 0)^T$
%respectively, we get the signature $f_6$ whose signature matrix is
%$M(f_6)=\left[\begin{smallmatrix}
%1 & 0 & 0 & \frac{d}{b}\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%-\frac{b}{d} & 0 & 0 & -1\\
%\end{smallmatrix}\right]$.
%By connecting two copies of $f_6$, we get the signature $f_7$ whose signature matrix is
%\[M(f_7)=M(f_6)NM_{x_3x_4, x_1x_2}(f_6)=\left[\begin{smallmatrix}
%1 & 0 & 0 & \frac{d}{b}\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%-\frac{b}{d} & 0 & 0 & -1\\
%\end{smallmatrix}\right]N\left[\begin{smallmatrix}
%1 & 0 & 0 & -\frac{b}{d}\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%\frac{d}{b} & 0 & 0 & -1\\
%\end{smallmatrix}\right]=2\left[\begin{smallmatrix}
%\frac{d}{b} & 0 & 0 & -1\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%-1 & 0 & 0 & \frac{b}{d}
%\end{smallmatrix}\right].\]
%By Lemma~\ref{normalize:a=x}, we can assume that $f_7$ has the signature matrix $M(f_7)=\left[\begin{smallmatrix}
%1 & 0 & 0 & -1\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%-1 & 0 & 0 & 1
%\end{smallmatrix}\right]$.
%Then by connecting two copies of $f_7$, we get the signature $f_8$ whose signature matrix is
%\[
%M(f_7)NM(f_7)=\left[\begin{smallmatrix}
%1 & 0 & 0 & -1\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%-1 & 0 & 0 & 1
%\end{smallmatrix}\right]N\left[\begin{smallmatrix}
%1 & 0 & 0 & -1\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%-1 & 0 & 0 & 1
%\end{smallmatrix}\right]=2\left[\begin{smallmatrix}
%-1 & 0 & 0 & 1\\
%0 & 1 & 1 & 0\\
%0 & 1 & 1 & 0\\
%1 & 0 & 0 & -1
%\end{smallmatrix}\right].
%\]
%Note that Holant$(\neq_2|f_8, (0, 1, 2, 0)^T)\geq_{T}\leq_T^p$Holant$(\neq_2|f, (0, 1, t, 0)^T)$.
%We finish the proof by proving that  Holant$(\neq_2|f_8, (0, 1, 2, 0)^T)$ is \#P-hard.
%Let $T=\left[\begin{smallmatrix}
%1 & i\\
% i & 1
%\end{smallmatrix}\right]$. By the holographic transformation using $T$, we have
%\[
%\operatorname{Holant}(\neq_2|f_8, (0, 1, 2, 0)^T)\equiv_{T}\operatorname{Holant}(\neq_2|=_4, g),
%\]
%where $g=(3, \frak{i}, -\frak{i}, 3)^T$.
%By Lemma~\ref{equality-4-csp2}, we have
%\[
%\operatorname{\#CSP}^2(g)\leq_T^p\operatorname{Holant}(\neq_2|=_4, (3, \frak{i}, -\frak{i}, 3)^T).
%\]
%Since $g\notin\mathscr{P}\cup\mathscr{A}\cup\alpha\mathscr{A}\cup\mathscr{L}$, \#CSP$^2(g)$ is \#P-hard by Theorem~\ref{CSP2}.
%Thus Holant$(\neq_2|f_8, (0, 1, 2, 0)^T)$ is \#P-hard.%
%\item For $\frac{by}{dw}=1$, note that the inner matrix of $M_{x_1x_3, x_2x_4}(f_1)=\left[\begin{smallmatrix}
%a & 0 & 0 & 1\\
%0 & \frac{b}{d} & 1 & 0\\
%0 & 1 & \frac{y}{w} & 0\\
%-1 & 0 & 0 & \frac{a}{dw}
%\end{smallmatrix}\right]$ is degenerate.
%The remaining proof is similar with the case that $\frac{by}{dw}=-1$ and we omit it here.
%\end{itemize}
%\fi%


==> 7ref-s.tex <==

\begin{thebibliography}{50}
\bibitem{ahlfors}Ahlfors, L., Complex Analysis, 3 ed. (McGraw-Hill, 1979).

%%%%%%%%%%%%%%%%%%%%
\bibitem{Beckens-arXiv} Miriam Backens.
A new Holant dichotomy inspired by quantum computation.
https://arxiv.org/pdf/1702.00767.pdf.

\bibitem{Bulatov}
Andrei A. Bulatov:
The Complexity of the Counting Constraint Satisfaction Problem. ICALP (1) 2008: 646-661.

\bibitem{1-below-Bulatov-Dalmau}
A. A. Bulatov and V. Dalmau, Towards a dichotomy theorem for the counting constraint satisfaction problem, Inform. and Comput., 205 (2007), pp. 651--678.

\bibitem{2-below}
A. Bulatov, M. Dyer, L. A. Goldberg, M. Jalsenius, M. Jerrum, and D. Richerby, The complexity of weighted and unweighted \#CSP, J. Comput. System Sci., 78 (2012), pp. 681--688.

\bibitem{Bulatov-Grohe}Andrei A. Bulatov, Martin Grohe:
The complexity of partition functions. Theor. Comput. Sci. 348(2-3): 148-186 (2005).



%%%%%%%%%%%%%%

\bibitem{Cai-Chen-generalCSP}
Jin-Yi Cai, Xi Chen:
Complexity of counting CSP with complex weights. STOC 2012: 909-920.

\bibitem{Cai-Chen-Lu-forGH}
Jin-Yi Cai, Xi Chen, Pinyan Lu:
Graph Homomorphisms with Complex Values: A Dichotomy Theorem. SIAM J. Comput. 42(3): 924-1029 (2013).

\bibitem{Cai-Chen-Lu-for-nonnegative-general-domain-CSP}
Jin-Yi Cai, Xi Chen, Pinyan Lu:
Nonnegative Weighted \#CSP: An Effective Complexity Dichotomy. SIAM J. Comput. 45(6): 2177-2198 (2016).





\bibitem{cai:chen:ll} Jin-Yi Cai, Xi Chen, Richard J. Lipton, and Pinyan Lu. On tractable exponential sums. In FAW, pages
148-159. Springer Berlin Heidelberg, 2010.
\bibitem{cai:fu:plcsp} Jin-Yi Cai, Zhiguo Fu:
Holographic Algorithm with Matchgates Is Universal for Planar $\#$CSP Over Boolean Domain. CoRR abs/1603.07046 (2016).

\bibitem{cai-fu-guo-williams}Jin-Yi Cai, Zhiguo Fu, Heng Guo, Tyson Williams:
A Holant Dichotomy: Is the FKT Algorithm Universal? FOCS 2015: 1259-1276.

\bibitem{cai:fu:xia} Jin-Yi Cai, Zhiguo Fu, Mingji Xia:  Complexity Classification Of The Six-Vertex Model.
https://arxiv.org/abs/1702.02863.

\bibitem{caiguowilliams13}Jin-Yi Cai, Heng Guo, Tyson Williams:
A complete dichotomy rises from the capture of vanishing signatures: extended abstract. STOC 2013: 635-644.

\bibitem{cai-huang-lu}Jin-Yi Cai, Sangxia Huang, Pinyan Lu:
From Holant to \#CSP and Back: Dichotomy for Holant c Problems. Algorithmica 64(3): 511-533 (2012).

\bibitem{cailuxiastar}Jin-Yi Cai, Pinyan Lu, Mingji Xia:
Dichotomy for Holant* Problems with Domain Size 3. SODA 2013: 1278-1295

\bibitem{cailuxia-2014}Jin-Yi Cai, Pinyan Lu, Mingji Xia:
The complexity of complex weighted Boolean \#CSP. J. Comput. Syst. Sci. 80(1): 217-236 (2014).

\bibitem{cailuxia-2017}Jin-Yi Cai, Pinyan Lu, Mingji Xia:
Dichotomy for Real Holantc Problems.
https://arxiv.org/abs/1702.02693.



\bibitem{Dyer-Greenhill}Martin E. Dyer, Catherine S. Greenhill:
The complexity of counting graph homomorphisms. Random Struct. Algorithms 17(3-4): 260-289 (2000).

\bibitem{Dyer-Richerby}Martin E. Dyer, David Richerby:
An Effective Dichotomy for the Counting Constraint Satisfaction Problem. SIAM J. Comput. 42(3): 1245-1274 (2013).

\bibitem{Goldberg-Jerrum-Grohe-Thurley}
Leslie Ann Goldberg, Martin Grohe, Mark Jerrum, Marc Thurley:
A Complexity Dichotomy for Partition Functions with Mixed Signs. SIAM J. Comput. 39(7): 3336-3402 (2010).


\bibitem{huang-lu-2016}
Sangxia Huang, Pinyan Lu:
A Dichotomy for Real Weighted Holant Problems. Computational Complexity 25(1): 255-304 (2016).

\bibitem{tutte}Michel Las Vergnas:
On the evaluation at (3, 3) of the Tutte polynomial of a graph. J. Comb. Theory, Ser. B 45(3): 367-372 (1988).

\bibitem{wang-lin-2016}Jiabao Lin, Hanpin Wang:
The Complexity of Holant Problems over Boolean Domain with Non-negative Weights. CoRR abs/1611.00975 (2016).

\bibitem{Val08} Leslie G. Valiant: Holographic Algorithms. SIAM J. Comput. 37(5): 1565-1594 (2008).




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{thebibliography}


